Distributed Scenario-Based Optimization for Asset Management in a Hierarchical Decision Making Environment

Asset management attempts to keep the power system in working conditions. It requires much coordination between multiple entities and long term planning often months in advance. In this work we introduce a mid-term asset management formulation as a stochastic optimization problem, that includes three hierarchical layers of decision making, namely the mid-term, short-term and real-time. We devise a tractable scenario approximation technique for efficiently assessing the complex implications a maintenance schedule inflicts on a power system. This is done using efficient Monte-Carlo simulations that trade-off between accuracy and tractability. We then present our implementation of a distributed scenario-based optimization algorithm for solving our formulation, and use an updated PJM 5-bus system to show a solution that is cheaper than other maintenance heuristics that are likely to be considered by TSOs.

==> 221/ID2.2.1+real-time+operation.tex <==
%!TEX root =  ID2.2.1.tex
\section{Introduction}

\label{sec: intro}


This  chapter discusses the mathematical formulation of reliability criteria and optimization problems concerning the steady-state real-time operation. To set the background, we recall  from GARPUR D2.1 that:\\

%\emph{``


%\textbf{Power system reliability} is the probability that an electric power system can perform a required function under given conditions for a given time interval. Reliability quantifies the ability of an electric power system to supply adequate electric service on a nearly continuous basis with few interruptions over an extended period of time.}\\

%\emph{
%A \textbf{reliability criterion} is a principle imposing a standard to determine whether or not the reliability level of a power system is acceptable. On the basis of a formal approach of decision-making at TSO level, a tentative (probabilistic or deterministic) reliability criterion (RC) can be seen as part of the constraints and cost functions of an optimisation problem.}\\

%\emph{\textbf{Reliability management} means to take a sequence of decisions under uncertainty. It aims at meeting a reliability criterion while minimizing the socio-economic costs of doing so.\\}

\emph{``\textbf{Real-time operation} is exercised within recurring time intervals, beginning with a regular update on the system operating conditions. The duration of these intervals (typically in the range of 15 -- 60 minutes) is such that the system operating conditions can be assumed to be relatively predictable, unless a contingency happens. Real-time operation includes preventive, corrective and emergency operation.''\\}

%In the remainder of this note, we discuss the mathematical formulation of alternative reliability criteria as parts of constraint and objective functions of optimization problem statements, \textit{i.e.} reliability management decision making problems. 

We begin in section \ref{sec:rtprev} by  introducing the alternative reliability criteria and optimization problems in the context of only preventive operation, while neglecting corrective control and it's failure probability. Subsequently, section \ref{sec:theother} expands these in the context of preventive/corrective operation.






\section{Real-time preventive operation}
\label{sec:rtprev}

\subsection{Preliminaries}

 Without loss in generality, we consider the simple set-up of real-time preventive operation only, as shown in Figure \ref{fig:rt_ovrw}. 



\begin{figure}[h]

\begin{framed}
\centering
\begin{tabular}{ccc}
&&\\
\textbf{\emph{Select \& apply}}&&\\
$\mathbf{u_0} \in \mathcal{U}_0(x_0,y_0) $		&&$\circ$\\
$\downarrow$&	$\nearrow$&.	\\	 
{$\bullet $}&$\pi_c \rightarrow $ &.\\
$x_0$&$\searrow$& .\\
&&$\circ$\\
&$ c \in \mathcal{N} $ &$x_c(x_0,u_0,y_c) $\\
\multicolumn{3}{c}{$\dotfill$}\\
\multicolumn{3}{c}{$\textbf{\emph{Assess \& minimize}}$}\\
\multicolumn{3}{c}{$\dotfill$}\\
$\downarrow$&&$\downarrow$\\
$C_0(x_0,u_0,y_0) \ge 0$&&$c_{R}(x_c,u_0,y_c)\ge 0$\\
&&\\
\hline
\end{tabular}
\\

\small{
\begin{description}
\item[$\mathbf{x}$]{is a vector  of state variables (voltage magnitude \& angle at all network nodes); }
\item[$\mathbf{y}$]{is a vector of all exogenous parameters (\textit{e.g} transmission line ratings, cost coefficients, component outages per event $(c)$ \textit{etc.}.); }
\end{description}

}

\end{framed}
\caption{Real-time preventive operation}
\label{fig:rt_ovrw}

\end{figure}


In the set-up of fig. \ref{fig:rt_ovrw}, reliability management consists of selecting  decisions $u_0 \in \mathcal{U}_0(x_0,y_0) $ (\textit{e.g.,} active power generation re-dispatch with respect to a market outcome, breaker statuses, \textit{etc.}) to apply prior to the realization of the uncertainty. We consider that  uncertainty can be characterized by a finite set of mutually exclusive and collectively exhaustive events\footnote{We recall that any two events are mutually exclusive if they cannot occur jointly. Moreover, a set of events is collectively exhaustive if at least one of these events must occur. Thus, in the context of real-time operation set $\mathcal{N}$ would include the pseudo-contingency of normal operation, single outages as well as higher order outages.} $(\mathcal{N})$. Denoting the probability of elementary event $c \in \mathcal{N}$ as $(\pi_c)$, we have $\sum_{c \in\mathcal{N}} \pi_c = 1$.  Selecting any decision  $u_0 \in \mathcal{U}_0(x_0,y_0) $ would result in monetary costs measured by \emph{cost function} $C_0(x_0,u_0,y_0)$. Upon the  realization of any event $c \in \mathcal{N}$, resulting in the realized system state $x_c(x_0,u_0,y_c)$, \emph{criticality function} $c_R(x_c,u_0,y_c) \ge 0$ expresses in monetary terms  the consequences of a potential service interruption sustained by the system end-users. 


In the remainder of this section we discuss the formulation of reliability criteria and optimization problem statements in the set-up presented in Fig. \ref{fig:rt_ovrw}. We maintain as a basis the unconstrained minimization of the compound expectation of monetary costs and consequences of service interruptions, 

\begin{flalign}
\min_{u_0 \in \mathcal{U}_0(x_0,y_0)}& W(x_0,u_0, \mathcal{N})= \left(C_0(x_0,u_0,y_0)+ \sum_{c \in\mathcal{N}} \pi_c \cdot c_R(x_c,u_0,y_c) \right). & \label{ideal}
\end{flalign}

We note that the second term in \eqref{ideal} measures the risk of service interruption to the system end-users as a summation of the product of the probability and criticality of all collectively exhaustive events. In a theoretical context and provided that criticality function $ c_R(x_c,u_0,y_c) $ accurately measures the societal impact of electricity service interruption (integrating, if relevant,  considerations of risk aversion, distributional considerations, effects of time, duration and geographical extent of interruptions on the consumer utility loss, \textit{etc.}) it can be argued that expression \eqref{ideal} is equivalent to the mathematical formulation maximizing the welfare of the electricity system stakeholders\footnote{It is important to underline here that, in the set-up of real-time operation minimizing the total costs \eqref{ideal} is equivalent to maximizing the benefits, since the terms cost and benefit are antonyms. We refer the interested reader to GARPUR ID3.2.1 for a comprehensive discussion on the terms of this function.}.


\subsection{The N-1 Criterion}
\label{sec:N-1}


\emph{``The N-1 criterion is a principle according to which the system should be able to withstand at all times a credible contingency --\textit{ i.e.}, unexpected failure or outage of a system component (such as a line, transformer, or generator -- in such a way that the system is capable of accommodating the new operational situation without violating operational security limits.''\\}


As a starting point, we sketch the mathematical formulation of the currently applicable N-1 criterion and establish it's relation to \eqref{ideal}. This criterion is theoretically based on the premise that all elementary events apart from the normal operation and the outage/failure of any single component have a negligible probability\footnote{In practice, the premise is followed in an ad-hoc manner leading to several possible interpretations of the term ``N-1 criterion''.  }. Defining $\mathcal{N}_{-1} \subset \mathcal{N}$  as the subset containing the event of normal operation and all single component outages/failures, the basic premise of the N-1 criterion can be stated as,

\begin{flalign}
\sum_{c \in\mathcal{N}\setminus \mathcal{N}_{-1}} \pi_c   \approx 0 \Rightarrow \sum_{c \in\mathcal{N}_{-1}} \pi_c   \approx 1.&&\label{N-1proba}
\end{flalign}

The premise stated in \eqref{N-1proba} may also imply that the summation of the product of probability times criticality for all events outside the subset $\mathcal{N}_{-1}$ can also be considered as negligible, irrespectively of the chosen decision $u_0 \in \mathcal{U}_0(x_0,y_0)$, \textit{i.e.},

\begin{flalign}
\sum_{c \in\mathcal{N}\setminus{N}_{-1}} \pi_c \cdot c_R(x_c,u_0,y_c)  \approx 0 \quad \forall u_0 \in \mathcal{U}_0(x_0,y_0).&&
\end{flalign} 

Under such conditions one can approximate \eqref{ideal} by


\begin{flalign}
\min_{u_0 \in \mathcal{U}_0(x_0,y_0)}& \left( C_0(x_0,u_0,y_0)+ \sum_{c \in\mathcal{N}_{-1}} \pi_c \cdot c_R(x_c,u_0,y_c) \right).  &\label{n-1step}
\end{flalign}

Over this subset of events, the N-1 criterion can be expressed as a set of technical constraints on the decision and network state variables (including Kirchoff's laws, limits on equipment ratings, dynamic constraints,  the requirement that the total consumer demand should be served under any system state, \textit{etc.}). Denoting such constrains via function $h(x_c,u_{0},y_c)$, the problem corresponding to the N-1 criterion can be compactly stated as, 




\begin{flalign}
\min_{u_0 \in \mathcal{U}_0(x_0,y_0)}& \left( C_0\left(x_0,u_0,y_0\right)+ \sum_{c \in\mathcal{N}_{-1}} \pi_c \cdot c_R(x_c,u_0,y_c) \right)  & \label{rtn-1.1}\\
s.t.&&\nonumber\\
&h(x_c,u_{0},y_c) \le  0\quad\forall c \in \mathcal {N}_{-1}.\label{rtn-1.2}
\end{flalign} 


We notice that the second term in \eqref{rtn-1.1}, corresponding to the expectation of the consequences of service interruption under all events within set $\mathcal{N}_{-1}$ appears redundant, as the set of constraints \eqref{rtn-1.2} imposes that there should be no service interruption under any such event. 
Indeed, constraint set \eqref{rtn-1.2} is equivalent to a set of constraints restricting criticality to zero for all events within subset $\mathcal{N}_{-1}$, as in,

\begin{flalign}
h(x_c,u_0,y_c)\le 0 \equiv c_{R}(x_c,u_0,y_c) = 0 \quad \forall c \in \mathcal{N}_{-1}, &&\\
\intertext{or, more generally,}
h(x_c,u_0,y_c)\le 0 \equiv c_{R}(x_c,u_0,y_c) \le \bar{c}_R \quad \forall c \in \mathcal{N}_{-1} & \quad (with\quad \bar{c}_R=0).&\nonumber
\end{flalign}


 It follows that constraint set \eqref{rtn-1.2} enforces $\sum_{c \in\mathcal{N}_{-1}} \pi_c \cdot c_R(x_c,u_0,y_c) = 0 \quad \forall u_0 \in \mathcal{U}_0(x_0,y_0)$, hence the problem corresponding to the N-1 criterion is commonly stated as, 


\begin{flalign}
\min_{u_0 \in \mathcal{U}_0(x_0,y_0)}& C_0\left(x_0,u_0,y_0\right) & \label{rtn-21.1}\\
s.t.&&\nonumber\\
&h(x_c,u_{0},y_c) \le  0\quad \forall c \in \mathcal {N}_{-1}.\label{rtn-21.2}
\end{flalign} 

We underline here that since constraint \eqref{rtn-21.2} is only considered over the subset $\mathcal{N}_{-1}\subset \mathcal{N}$, the N-1 criterion only limits the consequences of a potential service interruption  at least with a probability of  $\sum_{c \in \mathcal{N}_{-1}} \pi_c \le 1$. The N-1 criterion is thus a particular instance of the chance constrained formulation\footnote{where we use the following notation to denote probability,
\begin{flalign}
&\mathbb{P}_{c \in \mathcal{N}}  \left( \alpha(c) \le \beta\right) \equiv \sum_{c \in \mathcal{N}}\pi_c  \cdot  \mathbf{1}_{\{\alpha(c) \le \beta\}}&\\
& \mathbf{1}_{\{\alpha(c) \le \beta\}}\equiv  \left\{  \begin{array}{l}
  1 \quad if \quad \alpha(c) \le \beta \\
0 \quad else.   \end{array} 		\right. &&
\end{flalign}}
,



\begin{flalign}
\min_{u_0 \in \mathcal{U}_0(x_0,y_0)}&\left( C_0(x_0,u_0,y_0)+ \sum_{c \in\mathcal{N}} \pi_c \cdot c_R(x_c,u_0,y_c) \right)  &\label{c.chance}\\
s.t.&&\nonumber\\
&\mathbb{P}  \left( h(x_c,u_0,y_c) \le 0 \right) \geq  \sum_{c \in \mathcal{N}_{-1}} \pi_c.  &\label{c.chance2}\\
\intertext{\textbf {under the assumption that}}
&\sum_{c \in\mathcal{N}\setminus\mathcal{N}_{-1}} \pi_c \cdot c_R(x_c,u_0,y_c)  \approx 0 \quad \forall u_0 \in \mathcal{U}_0( x_0,u_0). &
\end{flalign}



\subsection{Towards the formulation of alternative  reliability criteria}


As established in the precedent paragraphs, the use of the N-1 criterion can be interpreted as a particular way of approximating the unconstrained minimization of the compound expectation of monetary costs and consequences of service interruptions \eqref{ideal}.  Indeed, the unconstrained minimization of the compound expectation of monetary costs and consequences of service interruptions can be practically unattainable, particularly due to the following challenges:

\begin{enumerate}[(i)]
\item{the cardinality of the set of  mutually exclusive and collectively exhaustive events $\mathcal{N}$ can be too large;}
\item{modeling in the time domain the dynamic trajectories induced by the occurrence of any event $c \in \mathcal{N}$, given the choice of a decision $u_0 \in U_0(x_0,y_0)$ to optimize the transition $x_c(x_0,u_0,y_c)$ can be very complex. In practice, certain dynamic trajectories to be avoided at any cost can only be expressed as technical constraints along with objective function \eqref{ideal}; }
\item{an accurate model of  the criticality function $c_R(x_c,u_0,y_c)$ needed to  translate the technical characteristics of  service interruptions into a monetary value may not be determined for all possible realizations of $(x_c,u_0,y_c)$.}
\end{enumerate}

On this basis, we discuss here the formulation of alternative reliability criteria, generalizing the principles of the N-1 criterion, towards more accurate approximations of \eqref{ideal}. 



\subsubsection{Defining a subset of credible events}
\label{subsec:Cred}

Since the set of mutually exclusive and collectively exhaustive events $\mathcal{N}$ may be too large in any practical context, 
we consider  the definition of a subset of credible events $\mathcal{N}_c \subset \mathcal{N}$ to approximate the reliability management problem in \eqref{ideal} as, 

\begin{flalign}
\min_{u_0 \in \mathcal{U}_0(x_0,y_0)}&  W(x_0,u_0, \mathcal{N}_c)= \left(C_0(x_0,u_0,y_0)+ \sum_{c \in\mathcal{N}_c} \pi_c \cdot c_R(x_c,u_0,y_c) \right). & \label{obj.subset}
\end{flalign}


Given any such subset $\mathcal{N}_c$, let  $(u_0^{\star}|\mathcal{N}_c)$ denote an optimal solution to \eqref{obj.subset}, as in, 
\begin{flalign}
(u_0^{\star}|\mathcal{N}_c)\equiv u^{\star}_0  \in \argmin_{u_0 \in \mathcal{U}_0(x_0,y_0)}  W(x_0,u_0, \mathcal{N}_c).&&\end{flalign}

We begin by noting that considering  any subset $\mathcal{N}_c \subset \mathcal{N}$ as opposed to the complete set $\mathcal{N}$   yields a residual risk $R_{\mathcal{N}\setminus \mathcal{N}_c} (u_0^{\star}|\mathcal{N}_c) $\footnote{In order to ease notation, the dependence of residual risk on the system state $x_0$ as well as on the problem parameters is left implicit.}, associated to the possible occurrence of any event outside this subset:



%R_{\mathcal{N}\setminus \mathcal{N}_c} 


\begin{flalign}
& R_{\mathcal{N}\setminus \mathcal{N}_c} (u_0^{\star}|\mathcal{N}_c)  = \sum_{c \in \mathcal{N}\setminus \mathcal{N}_c} \pi_c \cdot c_R(x_c,u^{\star}_0,y_c),&  \\
\intertext{with}
&\min_{u_0 \in \mathcal{U}_0(x_0,y_0)}  W(x_0,u_0, \mathcal{N}_c) +R_{\mathcal{N}\setminus \mathcal{N}_c} (u_0^{\star}|\mathcal{N}_c)  \ge \min_{u_0 \in \mathcal{U}_0(x_0,y_0)} W(x_0,u_0, \mathcal{N}). &
\end{flalign}




For a chosen subset $\mathcal{N}_c \subset \mathcal{N}$,  the residual risk value measures the quality of approximating the expectation of consequences of service interruption as, 

\begin{flalign}
& R_{\mathcal{N}\setminus \mathcal{N}_c} (u_0^{\star}|\mathcal{N}_c)  \approx 0& \label{waves}\\
 \Rightarrow &\sum_{c \in \mathcal{N}_c}\pi_c \cdot c_R(x_c,u_0^{\star}|\mathcal{N}_c,y_c) \approx   \sum_{c \in \mathcal{N}}\pi_c \cdot c_R(x_c,u_0^{\star}|\mathcal{N}_c,y_c). &
\end{flalign}


%\begin{flalign}
%& R_{\mathcal{N}\setminus \mathcal{N}_c} (u_0^{\star}|\mathcal{N}_c)  \approx 0& \label{waves}\\
% \Rightarrow &\argmin_{u_0 \in \mathcal{U}_0(x_0,y_0)} \sum_{c \in \mathcal{N}_c}\pi_c \cdot c_R(x_c,u_0,y_c) \approx \argmin_{u_0 \in \mathcal{U}_0(x_0,y_0)}  \sum_{c \in \mathcal{N}}\pi_c \cdot c_R(x_c,u^{\star}_0,y_c). &
%\end{flalign}

This measure is naturally of interest when one seeks to define a subset of events  $\mathcal{N}_c \subset \mathcal{N}$. Moreover, the validity of  \eqref{waves} is an implicit assumption of the N-1 criterion. Towards the formulation of alternative reliability criteria, we propose to replace this implicit assumption with an explicit condition of the form,

\begin{flalign}
& R_{\mathcal{N} \setminus \mathcal{N}_c}(u_0^{\star}|\mathcal{N}_c)  \le \Delta E. & \label{condition} \end{flalign}

For a chosen accuracy limit $\Delta {E}$, condition \eqref{condition} leads to  a consistent formation of subsets $\mathcal{N}_c \subset \mathcal{N}$   while event probabilities \& consequences may change (\textit{e.g.,} across different real-time intervals). Such condition should result to a relaxed (with respect to the N-1) reliability criterion when possible, \textit{i.e.,}  when probabilities \& consequences of single outages can be neglected. Moreover, when necessary, \textit{ i.e.,} when probabilities \& consequences of higher order outages become important, condition \eqref{condition} should lead to a stronger criterion.

The choice of the accuracy limit $\Delta E$ is a practical consideration, addressing the aspect of computational complexity (in theory one would always wish to impose  $\Delta E = 0$). Moving towards greater values of $\Delta E $ should lead to less complex problem statements (reducing the cardinality of the set $\mathcal{N}_c$) at the expense of adopting a greater residual risk (increasing the right-hand side of \eqref{condition}). 


We  notice here that \eqref{condition} can only be exactly assessed given a subset $\mathcal{N}_c$ and once the corresponding vector of optimal decisions 
$(u_0^{\star}|\mathcal{N}_c)$ has been identified. We conclude by discussing three possible approaches for practically considering this condition in order to identify a subset of credible events relevant for reliability management, namely a pessimistic, an iterative and a hybrid approach.





\paragraph{Pessimistic Approach}

The idea of this approach is to avoid the (possibly complex) computation of the residual risk value as a function of the optimal vector of decision variables. Such computation may be considerably complex, not only since it requires solving for $(u_0^{\star}|\mathcal{N}_c)$ but also due to the need to exactly compute the criticality function value for all events outside the subset $\mathcal{N}_c$.

 While the latter computation may indeed be complex, we notice that  the maximum possible criticality function value, denoted henceforth as $(c_R^{max})$ should be in principle both known and defined irrespectively of the decision variable vector $(u_0)$. Rather, the greatest possible consequences of service interruption to the end-users should correspond to the  loss of the total utility of consuming electricity, which is defined according to the end-user characteristics only. Given a subset of events $\mathcal{N}_c$, an upper bound on the residual risk can thus be calculated as,




\begin{flalign}
& R_{\mathcal{N}\setminus \mathcal{N}_c} ^{max} = \sum_{c \in \mathcal{N}\setminus \mathcal{N}_c} \pi_c \cdot c_R^{max}=c_R^{max} \cdot(1- \sum_{c \in \mathcal{N}_c}\pi_c).&  \label{aprox.risk}
\end{flalign}



The pessimistic approach to defining a subset of credible events consists of:

\begin{enumerate}
\item{Adopting an accuracy limit $\Delta E$.}
\item{Finding the smallest subset of events such that $R_{\mathcal{N} \setminus \mathcal{N}_c}^{max}  \le \Delta E$. We note that, using \eqref{aprox.risk}, this condition can also be re-written as, 
\begin{flalign}
\sum_{c \in \mathcal{N}_c}\pi_c \ge 1- \frac{ \Delta E}{ c_R^{max}}.&&\label{fractals}\end{flalign} 
A trivial way to find the smallest subset satisfying \eqref{fractals} would be to start from an empty set and keep adding events in order of decreasing probability.

 } 
\item{Solving for $u^{\star}_0 \in \argmin_{u_0 \in \mathcal{U}_0(x_0,y_0)}  W(x_0,u_0, \mathcal{N}_c).$ }
\end{enumerate}




\paragraph{Iterative Approach}

The idea of this approach is to use \eqref{condition} in order to iteratively grow the sub-set of credible contingencies and identify an optimal vector of decision variables. Rather than using the approximation of the residual risk as in \eqref{aprox.risk}, one can compute the exact residual risk value after solving \eqref{obj.subset}. The results of this exact computation can be used to check whether \eqref{condition} holds, and, if not, to form a larger subset to resolve \eqref{obj.subset}. This approach amounts to:

\begin{enumerate}
\item{Adopting an accuracy limit $\Delta E$.}
\item{Forming an initial subset $\mathcal{N}_c^{k} \subset \mathcal{N}, \quad k=0$, \textit{e.g.,} by considering the larger probability events only.}
\item{Solving for $u^{\star,k}_0 \in \argmin_{u_0 \in \mathcal{U}_0(x_0,y_0)}  W(x_0,u_0, \mathcal{N}_c^k)$. }
\item{Computing the exact criticality value for all the  neglected events $c \in \mathcal{N}\setminus \mathcal{N}_c^k$. We must note that this step pre-supposes that, given a decision variable vector $(u_0^{\star}|\mathcal{N}_c^k)$, the computation of exact criticality values for all neglected events is  tractable. Here, we restrict to acknowledging that such computation is in general less complex than the cumbersome problem of optimizing \eqref{ideal} with respect to all events in the large(r) set $\mathcal{N}$. In the subsequent part of this note, we will discuss an alternative approach that can be used to provide an approximation in the case this exact computation of the criticality values appears intractable.}
\item{Checking whether condition \eqref{condition} holds.  }
\item{If not, expanding the subset $\mathcal{N}_c^{k+1}  \supset \mathcal{N}_c^{k} $, \textit{e.g.,} by including the events with the largest expected consequences, \textit{i.e.} largest product of probability times criticality.}
\end{enumerate}



\paragraph{Hybrid Approach}

A hybrid approach can be devised by combining the features of both the iterative and the pessimistic approach. As in the pessimistic approach, we maintain the intention of avoiding the laborious computation of the residual risk value as a function of the optimal vector of decision variables for all events outside the subset $\mathcal{N}_c$. Moreover, we also seek to reduce the conservativeness induced by the use of the $(c_R^{max})$ value to approximate the potential criticality of any such event. 


 A hybrid approach can combine features of both the iterative and pessimistic approaches by:


\begin{enumerate}
\item{Adopting an accuracy limit $\Delta E$.}
\item{Forming an initial subset $\mathcal{N}_c^{k} \subset \mathcal{N}, \quad k=0$, \textit{e.g.,} by considering the larger probability events only.}
\item{Solving for $u^{\star,k}_0 \in \argmin_{u_0 \in \mathcal{U}_0(x_0,y_0)}  W(x_0,u_0, \mathcal{N}_c^k)$. }
\item{Computing the exact criticality value only for a subset of the events $c \in \mathcal{N}\setminus \mathcal{N}_c^k$, \textit{e.g.,} for events of larger probability}.
\item{Using the maximum criticality value (as an approximation) for all other events, \textit{e.g.,} lower probability events.}
\item{Aggregating the residual risk value}.
\item{Checking whether condition \eqref{condition} holds.}
\item{If not, expanding the subset $\mathcal{N}_c^{k+1}  \supset \mathcal{N}_c^{k} $, \textit{e.g.,} by including the events with the largest product of probability and criticality.}
\end{enumerate}



\paragraph{Remark}

As a final remark on the question of defining a subset of credible events, we underline here that set $\mathcal{N}$ includes a pseudo-event corresponding to the case under which no contingency happens, \textit{i.e.,} to the normal system operation, distinguished henceforth by setting the index $(c=0)$. In consistency to the idea that it is both the probability and consequence, \textit{i.e.,} the risk, associated to any event that matters, we have so far avoided any differentiation regarding this event. We however note that, in general, the probability of such an event should be of the greatest order of magnitude.

 This implies that, under the pessimistic approach, such event should be among the first (if not the very first) to be included within subset $\mathcal{N}_c \subset \mathcal{N}$. While a similar argument cannot be directly made for the iterative or hybrid approach, we underline that under such approaches this event would only be excluded from subset $\mathcal{N}_c \subset \mathcal{N}$ in the occasion  that, for the chosen decision $(u_0^{\star}|\mathcal{N}_c)$, its associated risk appears negligible. Evidently, given the order of magnitude of the probability of this event, such condition can only be achieved if the consequences of this event are found to be negligible. In other words, excluding this event from subset  $\mathcal{N}_c \subset \mathcal{N}$ implies that it is found to be \emph{a priori} secure. 

Be that as it may, we acknowledge that one may wish to always be absolutely certain that the event corresponding to the normal operation remains within subset $\mathcal{N}_c$. To facilitate this, we notice that the ideas for defining subset $\mathcal{N}_c$ may also be considered while starting from the reduced set $\mathcal{N} \setminus (c=0)$, with an appropriate reconsideration of the value of the accuracy limit $\Delta E$. In this case, following the definition (through any of the approaches above) of an initial subset $\mathcal{N}_{c \ne 0}$, the complete subset $\mathcal{N}_c$ can be formed as $\mathcal{N}_{c} = \mathcal{N}_{c \ne 0} \cup (c=0) $.

Without loss in generality we henceforth consider that the event corresponding to normal operation is always included within the subset $\mathcal{N}_c$.


\subsubsection{Considering a criticality function}
\label{subsec:sev}

As previously argued, in addition to the size of the set $\mathcal{N}$, optimizing the expected consequences of service interruption may be practically challenging both due to the complex dynamics of the transition $x_0 \rightarrow x_c(x_0,u_0,y_c)$ and in the case that the evaluation of monetary impacts of some realizations of $(x_c,u_0,y_c)$ is not straightforward.

\paragraph{Given a subset $\mathcal{N}_c$}

 We begin by addressing this matter in progression with the preceding ideas, \textit{i.e.} by considering that one has indeed identified a subset of credible events $\mathcal{N}_c$ of acceptable size and residual risk, and focus on  the problem of identifying an optimal decision variable vector $(u^{\star}_0| \mathcal{N}_c)$, as in \eqref{obj.subset}. In such a context, we argue for the consideration of a set of technical constraints on the decision and state variables to overcome the above mentioned challenges. The reasoning to do so is twofold:


\begin{enumerate}[(i)]
\item{Such constraints can be used to restrict values of $(x_c,u_0,y_c)$ to realizations for which the dynamics of the transition $x_0 \rightarrow x_c(x_0,u_0,y_c)$ can be accurately computed. While this does not translate into the optimality of \eqref{obj.subset}, it ensures that the effects of all decisions are accurately represented in technical terms. This appears as a precondition in order to be able to make a sensible tradeoff between the monetary costs of strengthening reliability versus the consequences of service interruptions.  }
\item{Such constraints can also be used to restrict values of $(x_c,u_0,y_c)$ to realizations for which the criticality function $c_R(x_c,u_0,y_c)$ can accurately translate the technical characteristics of a service interruption into a monetary value. In a similar manner, this acts as a precondition for adopting  \eqref{obj.subset}.}

\end{enumerate}

We recall from Subsection \ref{sec:N-1} that a particular variant of this approach, using constraint function $h(x_c,u_0,y_c)\le 0,~ \forall c \in \mathcal{N}_{-1}$
 as equivalent to the constraint $c_R(x_c,u_0,y_c)= 0 \forall c \in \mathcal{N}_{-1}$,  is well embedded within the N-1 criterion.


\paragraph{Iteratively Growing a Subset $\mathcal{N}_c$}
%-- memo 4 me: take \epsilon or upper bound to make chance constraint ineffective

We now return to the fact that the computation of the criticality function value may also be relevant for defining the subset of credible events, as argued in section \ref{subsec:Cred}. Here, we discuss how constraint function $h(x_c,u_0,y_c)$ can be used for this computation either in the context of the iterative approach or of the hybrid approach.
%
We recall that, given an optimal decision vector $(u_0^{\star}| \mathcal{N}_c)$ this approach necessitates computing the values of $c_R(x_c,u^{\star}_0,y_c)$ for all (or at least, in the hybrid approach, some) events  $c\in \mathcal{N}\setminus \mathcal{N}_c$. For any such event, we have previously argued that the criticality value will only be exactly computable under the condition  ${h}(x_c,u^{\star}_0,y_c) \le 0$. Along these lines, it is possible to approximate the criticality value as, 

\begin{flalign}
& c_R(x_c,u^{\star}_0,y_c)  \left\{  \begin{array}{l}
 = c_R(x_c,u^{\star}_0,y_c) \quad \mbox{if} \quad {h}(x_c,u^{\star}_0,y_c) \le 0 \\
\approx c_R^{max}  \quad else   \end{array} 		\right. .  &  \label{sevapprox}
\end{flalign}


\subsection{Problem Statement}
We continue by presenting alternative formulations of the real-time preventive reliability management problem. Such formulations correspond to alternative reliability criteria, according to the precedent ideas. To this end, we maintain:

\begin{itemize}
\item{the consideration  of a subset $\mathcal{N}_c$, defined on the basis of accepting the residual risk this implies; and}
\item{the consideration of a constraint function ${h}(\dots)$, as an implicit upper bound on the possible consequences to the end-users.}
\end{itemize}


These ideas combined lead to a formulation of the real-time preventive reliability management problem as,

\begin{flalign}
\min_{u_0 \in \mathcal{U}_0(x_0,y_0)}& \left(C_0\left(x_0,u_0,y_0\right)+ \sum_{c \in\mathcal{N}_c} \pi_c \cdot c_R(x_c,u_0,y_c) \right) & \label{tec1.Repe}\\
s.t.&&\nonumber\\
&{h}(x_c,u_0,y_c) \le  0, ~\forall c \in \mathcal {N}_{c}\label{tec2.Repe}
\intertext{while}
&R_{\mathcal{N} \setminus \mathcal{N}_c}(u_0^{\star}|\mathcal{N}_c) \lw{\leq \Delta E}.  &
\end{flalign}

Once again, we notice that the set of constraints \eqref{tec2.Repe} constitutes a chance constraint over the uncertain variable $c \in \mathcal{N} \supset \mathcal{N}_c$. Accordingly, \eqref{tec1.Repe} -- \eqref{tec2.Repe} may also be stated as, 

\begin{flalign}
\min_{u_0 \in \mathcal{U}_0(x_0,y_0)}&\left( C_0\left(x_0,u_0,y_0\right)+ \sum_{c \in\mathcal{N}_c} \pi_c \cdot c_R(x_c,u_0,y_c) \right)& \label{t1.P}\\
s.t.&&\nonumber\\
&\mathbb{P}  \left( h(x_c,u_0,y_c) \le  0 \right)  \ge  \sum_{c \in \mathcal{N}_c}\pi_c& \label{t2.P}
\intertext{while}
&R_{\mathcal{N} \setminus \mathcal{N}_c}(u_0^{\star}|\mathcal{N}_c){\leq \Delta E}.  &
\end{flalign}




We argue here that imposing constraint \eqref{t2.P} may possibly lead to very conservative solutions, at the expense of increased monetary costs. We thus propose, for the sake of generality, to allow for the relaxation of  chance constraint \eqref{t2.P}, as in $\mathbb{P}  \left( h(x_c,u_0,y_c) \le  0 \right)  \ge (1-\varepsilon)\cdot \sum_{c \in \mathcal{N}_c}\pi_c$. The parameter $(\varepsilon)$ relaxes the probability threshold; while \eqref{t1.P} -- \eqref{t2.P} corresponds to the specific choice of $\varepsilon =0$. 


Finally, we once again turn our attention to the pseudo-event corresponding to the no-contingency case $(c=0)$. Acknowledging that one  may wish to  seek a firm guarantee on the consequences of this event, we propose the alternative formulation of \eqref{technical1.P33} - \eqref{technical3.P33}.




%\begin{framed}

\begin{flalign}
\min_{u_0 \in \mathcal{U}_0(x_0,y_0)}& \left(C_0\left(x_0,u_0,y_0\right)+ \sum_{c \in\mathcal{N}_c} \pi_c \cdot c_R(x_c,u_0,y_c)\right) & \label{technical1.P33}\\
s.t.&&\nonumber\\
& h(x_0,u_0,y_0) \le  0 &\label{technical2.P33}\\
&\mathbb{P}  \left( h(x_c,u_0,y_c) \le  0 \right)  \ge (1-\varepsilon)\cdot \sum_{c \in \mathcal{N}_{c\ne 0}}\pi_c& \label{technical3.P33}
\intertext{while}
&R_{\mathcal{N} \setminus \mathcal{N}_c}(u_0^{\star}|\mathcal{N}_c){\leq \Delta E}.  &
\end{flalign}
%\hrulefill
%\\
%\textbf{Reliability Criterion}
%\begin{itemize} 
%\item[{$\blacktriangleright$}]        an accuracy limit $ \Delta\mathbb{E} \Rightarrow \mathcal{N}_c :  R_{\mathcal{N} \setminus \mathcal{N}_c}(u_0^{\star}|\mathcal{N}_c)  \le \Delta E $,
%\item[{$\blacktriangleright$}]        an upper bound on criticality $\bar{c}_{R}\Rightarrow h_{\bar{c}_{R}}(\dots)$, and, 
%\item[{$\blacktriangleright$}]        a probability threshold $\varepsilon \in [0,1]$.
%\end{itemize}


%\end{framed}



 We recall from Section \ref{sec: intro} that in GARPUR D2.1 reliability is  defined as ``\emph{the probability that an electric power system can perform a required function under given conditions for a given time interval}''.

We notice that in \eqref{technical1.P33} - \eqref{technical3.P33} the required function to be performed by the system is expressed in mathematical terms as $ h(x_c,u_0,y_c) \le  0 $. As discussed earlier, this expression is in principle equivalent to imposing an upper bound on the criticality of service interruption, \textit{i.e.} to defining the required level of service to be provided by the system according to the actual criticalities of service interruptions. The precise definition of a required level of service is thus necessary to define both reliability and respectively reliability criteria. Following this, indeed the left-hand side of \eqref{technical3.P33} serves as a reliability indicator, since it expresses mathematicaly the probability of performing the specified function in the given time interval and range of operating conditions.

  Accordingly, expression \eqref{technical3.P33} constitutes the general format of alternative reliability criteria, with the right-hand side setting a limit on the acceptable value of this reliability indicator as per (a.)  the conditions corresponding to the set of events in the subset $\mathcal{N}_c$ and (b.) the threshold parameter $\varepsilon \in [0,1]$. Particular instances of such alternative reliability criteria can be specified through the definition of  parameters $(\Delta E, \varepsilon)$ and through the choice of a criticality threshold $\bar{c}_R \ge 0$ which can be impicitly or explicilty effective via function $ h(x_c,u_0,y_c)$. Evidently, such alternative reliability criteria can indeed be expressed as part of the constraints and objectives of an optimization problem, \textit{i.e.} as prescribed by GARPUR D2.1.






\section{Real-time preventive/corrective operation}
\label{sec:theother}

In the present section we expand the ideas previously discussed while acknowledging the option offered by corrective control actions. Acknowledging this option, the task of real-time reliability management consists of selecting:
\begin{enumerate}[(i)]
\item preventive control actions $u_0 \in \mathcal{U}_0(x_0,y_0)$ to be applied in anticipation of any event $c \in \mathcal{N}$; and
\item corrective control actions  $ u_c \in \mathcal{U}_c(x_0,u_0,y_c)$ to be applied upon realization of any event $c \in \mathcal{N}$. 
\end{enumerate}



In spite of the conceptual difference between preventive and corrective control actions, the former being applied beforehand and the latter activated only if a specific event happens, it is essential to underline that the selection between such options should happen at a common decision making point. Prior to the realization of any event $c \in \mathcal{N}$, preventive and corrective actions can be viewed as alternative options to achieve the objectives of reliability management. 

\subsection{Neglecting corrective control failure}

In order to facilitate the discussion,  we begin by neglecting the possible failure of corrective control and focus on the set-up presented in Fig.~\ref{fig:rtcorr_ovrw}.  As shown in this figure, the realization of any event $c \in \mathcal{N}$ would cause a  transition of $x_0 \rightarrow x_c(x_0,u_0,y_c)$, dependent on the applied preventive control actions $u_0 \in \mathcal{U}_0(x_0,y_0)$.  Pre-selected corrective actions ${u_c} \in \mathcal{U}_c(x_c,u_0,y_c) $	 may then be applied, at a cost of  $C_c(x_c,u_c,y_c) \ge 0$, resulting in a transition  $ x_c(x_0,u_0,y_c) \rightarrow x_c^0(x_0,u_0,y_c^0)  $.  

\begin{figure}[h]

\begin{framed}
\centering

\begin{tabular}{ccccc}
&&&&\\
\multicolumn{2}{c}{\emph{\textbf{Select \& apply}}}&$\mathbf{u_c} \in \mathcal{U}_c(x_c,u_0,y_c) $	&&\\
$\mathbf{u_0} \in \mathcal{U}_0(x_0,y_0) $	&&$\downarrow$	&&\\
$\mathbf \downarrow$&	$\nearrow$&$\bullet$&$\rightarrow$&$ \circ$	\\	 
{$\bullet $}&$\pi_c \rightarrow $ &.&$\rightarrow$&$ \circ$\\
$x_0$&$\searrow$&$\bullet$&$\rightarrow$&$ \circ$\\
&&$x_c(x_0,u_0,y_c) $&&$x_c^0(x_c,u_c,y_c^0)$ \\
&&&&\\
&\multicolumn{2}{c}{$ c \in \mathcal{N}$} &&\\
\multicolumn{5}{c}{$\dotfill$}\\
\multicolumn{5}{c}{$\textbf{\emph{Assess \& minimize}}$}\\
\multicolumn{5}{c}{$\dotfill$}\\
$\downarrow$&\multicolumn{2}{c}{$\downarrow$}&\multicolumn{2}{c}{$\downarrow$}\\
$C_0(x_0,u_0,y_0) $&\multicolumn{2}{c}{$C_c(x_c,u_c,y_c)$}&\multicolumn{2}{c}{$c_{R}(x_c^0,u_c,y_{c}^0)$}\\
&&&&\\
\end{tabular}


\end{framed}
\caption{Real-time preventive/corrective operation}
\label{fig:rtcorr_ovrw}

\end{figure}



\subsubsection{Defining a Subset of Credible Events}
\label{subsec:CorCred}


We discuss here the ideas of Section \ref{subsec:Cred} in the context of arbitrating between preventive and corrective control actions. 
We recall that the point of concern is that the set of all mutually exclusive and collectively exhaustive events $\mathcal{N}$ may be too large. Under this premise, 
sub-section \ref{subsec:Cred} presents three possible approaches for the identification of a subset $\mathcal{N}_c \subset \mathcal{N}$ to approximate the reliability management problem. We establish that these three approaches remain valid in the context of arbitrating between preventive and corrective control.

%, leading to approximations of \eqref{ideal_cc} as,  

%\begin{flalign}
%\min_{\mathbf{u} \in \mathcal{U}(x_0,y_0, \mathcal{N}_c)} W(x_0,\mathbf{u}, \mathcal{N}_c)= & \quad C_0(x_0,u_0,y_0)+ \sum_{c \in\mathcal{N}_c} %\pi_c \cdot C_c(x_o^c,u_c,y_c) & \nonumber\\
%& + \sum_{c \in\mathcal{N}_c} \pi_c \cdot \sum_{b \in \mathcal{N}_b(x_c^0,u_c,y_c)} \pi_b(x_0^c,u_c,y_c) \cdot sev(x_o^c,u_c,y_b)   \label{ideal_cc_approx}
%\end{flalign}

\paragraph{Pessimistic Approach}

The essence of the pessimistic approach  is to acknowledge that the greatest possible consequences of service interruption to the end-user are defined according to the end-user characteristics only, hence are independent of any real-time reliability management decision. On this basis, the pessimistic approach consists of identifying a subset $\mathcal{N}_c \subset \mathcal{N}$ such that, in the worst case, the residual risk value remains lower than a defined threshold. The resulting condition \eqref{fractals} is an expression of (i) the chosen accuracy limit, (ii) the maximum possible criticality value and (iii) the sum of the probabilities of all events in the subset $\mathcal{N}_c$. 

Evidently, all such parameters are defined independently of the available corrective control actions, hence the application of the pessimistic approach to the problem in question is straightforward. It is of course noteworthy that, in the general case, the availability of corrective control options constitutes a greater potential to counteract the consequences of any event $c \in \mathcal{N}$. It follows that in the question of preventive/corrective reliability management, the pessimistic approach introduces a greater degree of conservativeness with respect to the question of preventive only reliability management. 

\paragraph{Iterative Approach}

The computation of the residual risk value, given a subset $\mathcal{N}_c^k$ and the corresponding (preventive) decision $(u_0^{\star}|\mathcal{N}_c^{k})$ is the central concept in the iterative approach. We argue here that the option of corrective control does not provoke any change in such computation. To justify this argument, we recall that the question at hand is whether or not events in a  subset $\mathcal{N}\subset \mathcal{N}_c$ can be neglected in the statement of the reliability management problem without a considerable loss in accuracy of the corresponding objective function value. 

Assuming that any event $c \notin \mathcal{N}_c$ has indeed been neglected, we notice that the realization of this event would cause a transition of $x_0 \rightarrow x_c^0(x_0,u_0,y_c)$, which is  independent of corrective control. This is consistent with the fact that event $c \notin \mathcal{N}_c$ has been neglected  from the statement of the reliability management problem, hence no corrective control actions correspond to this event. It follows that events can only be neglected in the statement of the reliability management problem if the residual risk while taking no corrective actions is found to be acceptable. As a result, the iterative approach  can also be considered in the question of preventive/corrective reliability management.


\paragraph{Hybrid Approach}

The hybrid approach combines features of both the pessimistic and the iterative approach. Following the precedent arguments, it is straightforward to deduce that the hybrid approach is also directly applicable to the preventive/corrective reliability management question.


\subsection{Considering a criticality function}

We now turn to the consideration of a criticality function and follow-up on the ideas presented in Section \ref{subsec:sev}.

 In respect to this issue, we recall from sub-section \ref{subsec:sev} the argument that the criticality value is expressed as a function of state variables, decision variables and parameters $\left(c_R(x,u,y)\right)$. Moreover, the value of this function may only be computable for a  subset of  possible combined realizations of state variables, decision variables and parameters. Such a subset can be expressed by means of a set of constraints of the form ${h}(\dots) \le 0$ which implicitly imposes an upper bound of $\bar{c}_R$ on the criticality value. Accordingly, an approximate form of the criticality function can be expressed as, 


\begin{flalign}
& c_R(x,u,y)  \left\{  \begin{array}{l}
 = c_R(x,u,y) \quad \mbox{if} \quad {h}(x,u,y) \le 0 \\
\approx c_R^{max}  \quad else   \end{array} 		\right. .  &  \label{sevapprox_repe}
\end{flalign}

In the context of Fig.~\ref{fig:rtcorr_ovrw}, this implies the consideration of three sets of constraint functions corresponding to the no contingency operation \eqref{hnorm0}, the interval between the occurrence of a contingency event $(c \ne 0)$ and the application of corrective control actions \eqref{hpc}, and following the application of corrective actions \eqref{hpb}, as in,

\begin{flalign}
&{h}_{0}(x_0,u_0,y_0) \le 0 & \label{hnorm0}\\
&{h}_{PC}(x_c,u_0,y_c) \le 0,~ \forall c \in \mathcal{N}_{c \ne 0} \label{hpc}\\
&{h}_{C}(x_c^0,u_c,y_c^0) \le 0,~ \forall c \in \mathcal{N}_{c \ne 0}. \label{hpb}
\end{flalign}



We underline here that regarding the occurrence of any contingency event $(c \ne 0)$ both expressions \eqref{hpc} and \eqref{hpb} are necessary to express an equivalent to the constraint on the resulting criticality value when corrective control is considered. The former \eqref{hpc} describes the conditions under which corrective control may be applied. This corresponds, for instance, to the short-term thermal ratings of network components. The latter \eqref{hpb}, concerns the outcome of the application of corrective control actions.  



\subsubsection{Problem Statement}

Towards  extension of \eqref{technical1.P33} - \eqref{technical3.P33} for the preventive/corrective reliability management, while neglecting the possible failure of preventive control, we begin by discussing the notable changes in the problem statement. Such changes involve  the addition of a term in the objective function \eqref{prevcobj} to account for the potential cost of corrective control actions. Moreover,  the dependence of the feasible set of corrective actions $\mathcal{U}_c(x_c,u_0,y_c) $ on the chosen preventive decisions $u_0$ should be acknowledged \eqref{prevcoset}. Finally, as discussed earlier, three distinctive sets of technical constraint functions \eqref{hnorm22} -- \eqref{hpc22} should be used  as equivalent to an (implicit) upper bound on service interruptions. 	 




\begin{flalign}
\min_{\mathbf{u}} &\left[ C_0(x_0,u_0,y_0)+ \sum_{c \in\mathcal{N}_c} \pi_c \cdot \left(C_c(x_c,u_c,y_c)+c_R(x_c^0,u_c,y_c^0)\right)\right] & \label{prevcobj} \\
s.t.&&\nonumber\\
&\mathbf{u} \in \mathcal{U}(x_0,y_0,\mathcal{N}_c)\equiv
\left\{  \begin{array}{l}
u_0 \in \mathcal{U}_0(x_0,y_0),  \\
{u_c \in \mathcal{U}_c(x_0,u_0,y_c) \hspace{2mm} \forall c \in \mathcal{N}_c }  \end{array} 		\right\}   &  \label{prevcoset}\\
&{h}_{0}(x_0,u_0,y_0) \le 0 & \label{hnorm22}\\
& {h}_{PC}(x_c,u_0,y_c) \le 0 \quad \forall c \in \mathcal{N}_{c \ne 0} & \label{hpc21}\\
&  {h}_{C}(x_c^0,u_c,y_c^0) \le 0 \quad \forall c \in \mathcal{N}_{c \ne 0}, & \label{hpc22}
\intertext{while}
&R_{\mathcal{N} \setminus \mathcal{N}_c}(u_0^{\star}|\mathcal{N}_c){\leq \Delta E}.  &
\end{flalign}


We conclude by re-framing \eqref{prevcobj} -- \eqref{hpc22} in order to make the chance constraint, induced by the choice of subset $\mathcal{N}_c$, explicit and also allow for the consideration of the probability threshold $(\varepsilon)$.

\begin{flalign}
\min_{\mathbf{u}} & \left[ C_0(x_0,u_0,y_0)+ \sum_{c \in\mathcal{N}_c} \pi_c \cdot \left(C_c(x_c,u_c,y_c)+c_R(x_c^0,u_c,y_c^0)   \right)\right] & \\
s.t.&&\nonumber\\
&\mathbf{u} \in \mathcal{U}(x_0,y_0,\mathcal{N}_c)\equiv
\left\{  \begin{array}{l}
u_0 \in \mathcal{U}_0(x_0,y_0),  \\
u_c \in \mathcal{U}_c(x_0,u_0,y_c) \hspace{2mm} \forall c \in \mathcal{N}_c   \end{array} 		\right\}   & \\
&{h}_{0}(x_0,u_0,y_0) \le 0 & \label{hnorm}\\
&\mathbb{P}  \left( \begin{array}{l} {h}_{C}(x_c,u_0,y_c) \le 0  \\
\bar{h}_{PC}(x_c^{0},u_c,y_c^0) \le 0 \end{array} \right) \ge (1 - \varepsilon) \cdot \sum_{c \in\mathcal{N}_{c\ne 0}} \pi_c,  &
\intertext{while}
&R_{\mathcal{N} \setminus \mathcal{N}_c}(u_0^{\star}|\mathcal{N}_c){\leq \Delta E}.  &
\end{flalign}




\subsection{Acknowledging corrective control failure}


In the general case, the effect of  corrective control actions may not be fully predictable in advance. Rather,  for each three-tuple $(x_c^0,y_c,u_c)$, there may exist a set of possible corrective control behaviors, henceforth denoted as $\mathcal{N}_b(x_c^0,u_c,y_c)$. Assuming, for the sake of notational simplicity, that such set is discrete, the symbol $ \pi_b(x_0^c,u_c,y_c)$ denotes the probability of realization of any possible behavior  $b \in \mathcal{N}_b(x_c^0,u_c,y_c)$ with, $\sum_{b \in \mathcal{N}_b(x_c^0,u_c,y_c)} \pi_b(x_0^c,u_c,y_c) =1$. Acknowledging the possible failure of corrective control, the set-up of real-time reliability management is presented in  Fig. \ref{fig:rtcorf_ovrw}.


\begin{figure}[h]

\begin{framed}
\centering


\begin{tabular}{ccccc}
&&&&\\
\multicolumn{2}{c}{\emph{\textbf{Select \& apply}}}&$\mathbf{u_c} \in \mathcal{U}_c(x_c,u_0,y_c) $	&&\\
$\mathbf{u_0} \in \mathcal{U}_0(x_0,y_0) $	&&$\downarrow$	&&$\circ$\\
$\mathbf \downarrow$&	$\nearrow$&$\bullet$&$\nearrow$&.	\\	 
{$\bullet $}&$\pi_c \rightarrow $ &.&$\pi_b(x_c^0,u_c)\rightarrow $&.\\
$x_0$&$\searrow$&$\bullet$&$\searrow$& .\\
&&$x_c(x_0,u_0,y_c) $&&$\circ$\\
&&&\multicolumn{2}{c}{$x_c^b(x_c,u_c,y_c^b)$ }\\
&&&&\\
&\multicolumn{2}{c}{$ c \in \mathcal{N} $} &\multicolumn{2}{c}{$b \in \mathcal{N}_b(x_c,u_c)$}\\
\multicolumn{5}{c}{$\dotfill$}\\
\multicolumn{5}{c}{$\textbf{\emph{Assess \& minimize}}$}\\
\multicolumn{5}{c}{$\dotfill$}\\
$\downarrow$&\multicolumn{2}{c}{$\downarrow$}&\multicolumn{2}{c}{$\downarrow$}\\
$C_0(x_0,u_0,y_0) $&\multicolumn{2}{c}{$C_c(x_c,u_c,y_c)$}&\multicolumn{2}{c}{$c_{R}(x_c^b,u_c,y_{c}^b)$}\\
&&&&\\
\end{tabular}

\end{framed}
\caption{Real-time with corrective control failure}
\label{fig:rtcorf_ovrw}

\end{figure}


\subsubsection{Problem statement}

In the context of Fig.~\eqref{fig:rtcorf_ovrw}, both the expectation of the criticality function value as well as the set of constraints corresponding to the outcome of corrective control should be considered for all possible corrective control behaviors within the set $\mathcal{N}_b(x_c,u_c)$, as in  \eqref{fin_ob} and \eqref{hpc32} respectively. 


\begin{flalign}
 & C_0(x_0,u_0,y_0)+ \sum_{c \in\mathcal{N}_c} \pi_c \cdot C_c(x_c,u_c,y_c) + \sum_{c \in\mathcal{N}_c} \pi_c  { \sum_{b \in \mathcal{N}_b(x_c^0,u_c)}\pi_b(x_c^0,u_c) \cdot c_R(x_c^b,u_c,y_c^b) }  &\label{fin_ob}\\
& {h}_{PC}(x_c^b,u_c,y_c^b) \le 0 \quad \forall c \in \mathcal{N}_{c \ne 0}, \forall b \in \mathcal{N}_{b}(x_c,u_c)  & \label{hpc32}
\intertext{while}
&R_{\mathcal{N} \setminus \mathcal{N}_c}(u_0^{\star}|\mathcal{N}_c){\leq \Delta E}.  &
\end{flalign}

We underline here that constraint function \eqref{hpc32} covers all possible behaviors of corrective control, including the potential complete failure. In the latter case, constraint function \eqref{hpc32} becomes an expression of preventive decisions only. We must notice that selecting preventive decisions to satisfy this constraint function would make corrective control redundant. It follows that, in order to enable the use of corrective actions, constraint function \eqref{hpc32} would have to be relaxed. As already introduced, such a relaxation can be facilitated by the choice of a probability threshold $\varepsilon > 0 $. Taking this into account, we reframe the problem of real-time preventive/corrective reliability management as follows.






%\begin{framed}

\begin{flalign}
\min_{\mathbf{u}} &\left( C_0(x_0,u_0,y_0)+ \sum_{c \in\mathcal{N}_c} \pi_c \cdot C_c(x_c,u_c,y_c) \right) & \nonumber\\
&+ \sum_{c \in\mathcal{N}_c} \pi_c  { \sum_{b \in \mathcal{N}_b(x_c^0,u_c)}\pi_b(x_c^0,u_c) \cdot c_R(x_c^b,u_c,y_c^b) }  &\\
s.t.&&\\
&\mathbf{u} \in \mathcal{U}(x_0,y_0,\mathcal{N}_c)\equiv
\left\{  \begin{array}{l}
u_0 \in \mathcal{U}_0(x_0,y_0),  \\
u_c \in \mathcal{U}_c(x_0,u_0,y_c) \hspace{2mm} \forall c \in \mathcal{N}_c   \end{array} 		\right\}   & \\
&{h}_{0}(x_0,u_0,y_0) \le 0 & \label{h300}\\
&{\mathbb{P}\left( \begin{array}{l} {h}_{C}(x_c,u_0,y_c) \le 0  \\
{h}_{PC}(x_c^{b},u_c,y_c^b) \le 0 \end{array} \right) \ge (1 - \varepsilon)  \sum_{c \in\mathcal{N}_{c\ne 0}} \pi_c }~, &
\intertext{while}
&R_{\mathcal{N} \setminus \mathcal{N}_c}(u_0^{\star}|\mathcal{N}_c){\leq \Delta E}.  &
\end{flalign}



==> 221/ID2.2.1+short-term+planning.tex <==
%!TEX root =  ID2.2.1.tex

\section{Introduction}

\label{sec: intro}

This chapter discusses the mathematical formulation of reliability criteria and optimization problems  in the context of short-term operational planning. To set the background, we recall  from GARPUR D2.1 \cite{D2.1} Figure \ref{fig:D21planning}), illustrating that:\\


%\emph{``\textbf{Power system reliability} is the probability that an electric power system can perform a required function under given conditions for a given time interval. Reliability quantifies the ability of an electric power system to supply adequate electric service on a nearly continuous basis with few interruptions over an extended period of time.}\\
%
%\emph{
%A \textbf{reliability criterion} is a principle imposing a standard to determine whether or not the reliability level of a power system is acceptable. On the basis of a formal approach of decision-making at TSO level, a tentative (probabilistic or deterministic) reliability criterion (RC) can be seen as part of the constraints and cost functions of an optimisation problem.}\\
%
%\emph{\textbf{Reliability management} means to take a sequence of decisions under uncertainty. It aims at meeting a reliability criterion while minimizing the socio-economic costs of doing so.\\}

\emph{``\textbf{Operational planning} constitutes the preparatory phases before the reliability of a power system is realized throughout the real-time operation. The scope of operational planning is to apply actions that must be activated in advance in order to ensure that reliability management is achievable within a prolonged future period of time. Such period of time is denoted as an operational planning horizon and consists of a sequence of target real-time intervals.''\\} 

%
%Figure \ref{fig:D21planning},  adopted from GARPUR D2.1 \cite{D2.1}, illustrates the short-term operational planning decision timescales. As shown in this figure, operational planning decisions are typically made ahead of the start of the respective planning horizon. It follows that such decisions must be made under uncertainty on the particular instances of the reliability management problem to be tackled at each target real-time interval within the operational planning horizon. Subject to such uncertainty, the scope of short-term operational planning is to make decisions (\textit{e.g.} grid topology, scheduling of active/reactive power reserves, transmission capacity given to the markets -- see GARPUR D2.1 \cite{D2.1} and D6.1  \cite{D6.1}, for detailed lists of relevant decisions) in order to ensure that the real-time reliability management approach and criterion (RMAC) is achievable. 



\begin{figure}
\centering
\includegraphics[width=\textwidth]{D21_planning.jpg}
\caption{Short-term operational planning decision timescales. }
\label{fig:D21planning}
\end{figure}



\subsection{Preliminaries \& Notation}

Without loss in generality, we consider a single short-term operational planning decision making point (\textit{e.g.,} the day-ahead planning decision making point). We shall employ,


\begin{mydescription}{$\xi_{1,\dots,T} \in S$}

\item[$t \in {[1,T]} $]{as an index of real time intervals within the discrete set corresponding to the planning horizon;}
\item[$\xi_{t} $]{as a random exogenous\footnote{\textit{i.e.}, beyond the influence of the decision maker.} variable, using the convention that realization of $\xi_{t}$ is made at the start of the respective real-time interval  $t$;}
\item[$\xi_{1,\dots,T} \in S$]{as a unique scenario, \textit{i.e.} a sequence of random exogenous variables $\xi_t$, spanning the whole operational planning horizon $[1,T]$;}
\item[$\xi_{[1,t]}$]{to denote a history of already observed random variables, concerning  $[1,t]$;}

\item[$u_p \in \mathcal{U}_P$]{to denote a candidate operational planning decision and the respective set;} 
\item[$C_P(u_p)$]{as the function measuring the direct costs of any short-term operational planning decision.} 
\end{mydescription}


Referring the reader to \cite{D2.1} and \cite{D6.1} for lists of relevant short-term operational planning decisions, we recall that the said decisions affect the potential to achieve the real-time reliability management approach and criterion (RT-RMAC) during any target real-time interval within the planning horizon.  To ease notation, while underlining the dependence of the RT-RMAC on operational planning decisions made under uncertainty, in this chapter we denote by,


\begin{mydescription}{$W_{RT}\left(u_p,u_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right)$}
\item[$\pi_{c}(\xi_t) $ ]{the probability of realization of contingency $c \in \mathcal{N}(\xi_{t})$;}
\item[$u_{RT}(\xi_t)$]{a candidate real-time decision\footnote{Corresponding to (possibly several) selected preventive and/or corrective actions, to be applied at real-time interval $t$.} ;} 
\item[$\mathcal{U}_{RT}(u_p,u_{RT}(\xi_{[1,t-1]}),\xi_t)$]{the set of candidate real-time decisions;}%\footnote{The dependence of the set of real-time candidate decisions $\mathcal{U}_{RT}(u_p,\xi_t)$ on past real-time reliability management decisions is left implicit in the compact notation. At any real-time interval $t \in [1,T]$, the known history of uncertainty realizations $\xi_{1,\dots,t-1}$ and the RT-RMAC, correspond to a known history of past real-time decisions  $ u_{RT}^{\star}(\xi_{1,.\dots,t-1})$.  } for interval $t$;} 
\item[$\varepsilon_{RT}$]{the probability threshold of the RT-RMAC;}
\item[$\Delta E_{RT}$]{the accuracy limit of the RT-RMAC;}
\item[$h\left(u_p,\xi_t,u_{RT}(\xi_t)\right)$]{the constraint set to be satisfied in real-time;} 
\item[$c_{R}\left(u_p,\xi_t,u_{RT}(\xi_t), c\right)$]{the criticality function of the RT-RMAC;} 
\item[$W_{RT}\left(u_p,u_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right)$]{the objective function of the RT-RMAC.} 
\end{mydescription}

Accordingly, we will compactly state the RT-RMAC discussed in Chapter~\ref{chp:realtime} as the problem of choosing,

\begin{flalign}
 u^{\star}_{RT}(\xi_t) \in  \argmin_{u_{RT}(\xi_t)} &W_{RT}\left(u_p,u_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) & \label{comp.RT.obj}\\
&s.t.&\nonumber\\
&u_{RT}(\xi_t) \in \mathcal{U}_{RT}(u_p,u_{RT}(\xi_{[1,t-1]}),\xi_t)  & \label{comp.Uset} \\
&\mathbb{P}_{c \in \mathcal{N}_c (\xi_t) }  \left \{h\left(u_p,\xi_t,u_{RT}(\xi_t)\right)\le  0 \right \} \ge (1-\varepsilon_{RT}),& \label{comp.RT.chance}
\intertext{\textbf{while}}
\mathcal{N}_c(\xi_t) \subseteq \mathcal{N}(\xi_t):& \sum_{c \notin\mathcal{N}_c(\xi_t)} \pi_{c}(\xi_t) \cdot c_{R}\left(u_p,\xi_t,u^{\star}_{RT}(\xi_t), c \right)  \le \Delta{{E}_{RT}}.  &\label{comp.RT.risk}
\end{flalign}


Objective function \eqref{comp.RT.obj} corresponds to the summation of all relevant economic costs and expected criticality of service interruption, and particularly for a subset $\mathcal{N}_c(\xi_t)$ of negligible residual risk \eqref{comp.RT.risk}.  Expression \eqref{comp.Uset} formalizes the choice of decisions within the respective candidate set. Notice the dependence of the later on (i) short-term operational planning decisions ($u_p$), (ii) exogenous random variable ($\xi_t$) and, (iii) the sequences of precedent real-time reliability management decisions, defined according to the history of precedent observations $\left(u_{RT}(\xi_{[1,t-1]})\right)$ and the RT-RMAC.

We should also clarify that, in the compact notation, the left-hand side of \eqref{comp.RT.chance} denotes,

\begin{description}

\item[ $\mathbb{P}_{c \in \mathcal{N}_c (\xi_t) }  \left \{h\left(u_p,\xi_t,u_{RT}(\xi_t)\right)\le  0 ) \right \}$:]{the probability of achieving acceptable system performance  $\left(h\left(u_p,\xi_t,u_{RT}(\xi_t)\right)\le  0\right) $, subject to the uncertainty on the occurrence of contingencies $c \in \mathcal{N}_c(\xi_t)$ as well as the possible failure modes of corrective control (if applicable). The later is not explicitly represented here to ease notation.}
\end{description}

In this respect, \eqref{comp.RT.chance} serves to guarantee acceptable system performance with a given probability over the uncertainty on the occurrence of contingencies $c \in \mathcal{N}_c(\xi_t)$ and the possible post-contingency behaviors. Moreover, achieving \eqref{comp.RT.chance}, effectively achieves the following guarantee over the complete range of uncertainties $c \in \mathcal{N}(\xi_t)$,

\begin{flalign}
&\mathbb{P}_{c \in \mathcal{N}_c (\xi_t) }  \left \{h\left(u_p,\xi_t,u_{RT}(\xi_t)\right)\le  0 \right \} \ge (1-\varepsilon_{RT})\sum_{c \in \mathcal{N}_c(\xi_t)} \pi_c(\xi_t).& \label{comp.RT.chancefull}
\end{flalign}

We underline that \eqref{comp.RT.obj} -- \eqref{comp.RT.risk} is used here as a general formulation of a wide spectrum of reliability criteria. For example, as per the N-1 criterion the subset of negligible residual risk is defined to be the set of single outages, while the constraint set \eqref{comp.RT.chance} is to be satisfied with probability equal to one (\textit{i.e.}, for the no contingency case and under any single outage). Consequently, the expected criticality of service interruption would be equal to zero under all these events. 





\subsection{Chapter organization}

The remainder of this chapter is organised as follows. Section \ref{sec:unct} introduces a model of the uncertainty space $\xi_{1,\dots, T}$ as well as it's possible approximations. In Section~\ref{sec:ass}, we focus on the problem of assessing the implied consequences of a chosen operational planning decision $u_p \in \mathcal{U}_P$ and also identify possible approximations. Finally, we conclude in Section~\ref{sec:dec} by presenting the short-term operational planning reliability management approach and criterion. 


\clearpage


\section{Uncertainty modeling and its possible approximations}
\label{sec:unct}



The present section discusses \textbf{exogenous} uncertainty, as in  randomness outside the influence of the short-term operational planning decision maker. In other words, we focus here on uncertain factors  whose possible realizations may not be influenced by short-term operational planning decisions.
Rather, decisions may be taken in order to  be able to manage the system response to the possible realizations of the said uncertainty. 



 Recalling that the scope of short-term operational planning is to anticipate and prepare real-time operation, the matter of concern is the (yet unknown) instances of the real-time reliability management problems within the operational planning horizon. To be more specific, from the operational planning perspective, the following factors\footnote{we note that the factors mentioned here are indicative of the prominent considerations with regard to the operational planning uncertainty. Nevertheless, the discussion presented in this chapter is, in principle, applicable while acknowledging uncertainties of the real-time problem instance (\textit{e.g.}, weather dependent transmission line ratings).} may be modeled as functions of a random exogenous variable  $\xi_t \hspace{1mm} \forall t  \in [1,T]$ (as per the notation discussed in Section~\ref{sec: intro}), 

\begin{itemize}
\item[$\blacktriangleright$]{the (weather and possibly market dependent) nodal injections and demands;}
\item[$\blacktriangleright$]{the (weather dependent) failure rates, consequently failure probabilities, of network components; and} 
\item[$\blacktriangleright$]{the per unit costs of service interruption for the various classes of system end-users}.
\end{itemize}

We stress that a unique realization of random variable $\xi_t$  defines a single set of information corresponding to an instance of the real-time reliability management problem discussed in Chapter~\ref{chp:realtime} . Within such set of information, the uncertainty on the possible occurrence of contingencies (as well as failures of corrective control) remains still unresolved, to be tackled during the respective real-time interval. That is, a unique realization of random variable $\xi_t$, does not define the occurrence of a particular contingency within the respective real-time interval $t$. Rather, a unique realization of random variable $\xi_t$, would define the probabilities for all events within the discrete set $c \in\mathcal{N}(\xi_t)$, such that $\sum_{c \in\mathcal{N}(\xi_t)} \pi_c(\xi_t)=1$.

 Evidently, the uncertainty concerning the aforementioned factors is both  outside the influence of short-term operational planning decisions  and revealed in a sequential manner. The latter is,  at any $t \in [1,T]$ realizations onwards until the end of the operational planning horizon  $\xi_{t+1,\dots,T}$  remain unknown.   In the notation, we  shall follow the convention that the realization of the value of $\xi_t$ is only made at the start of the respective real-time interval $(t)$. 

\subsection{Possible Approximations}


\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{tree2.jpg}
\caption{Scenario tree approximation }
\label{fig:tree}
\end{figure}



From the general properties of random variable $\xi_{t}$ it is evident that the space of possible sequences of realizations spanning the whole operational planning horizon $\xi_{1,\dots,T} \in S$ becomes quite large to enumerate in practice as the span  $[1,T]$ increases.To tackle this issue, we propose to explore finite scenario approximations of the space $\xi_{1,\dots,T} \in S$. Referring the reader to \cite{dupacova,growe-kuska,defourny2012} for a comprehensive discussion on such approximations, we illustrate in figure \ref{fig:tree} the concept of a \emph{scenario tree}.


Each \emph{node} on the scenario tree of Figure~\ref{fig:tree} corresponds to a unique realization of random variable $\xi_t$ at the respective point in time. The leftmost  node is termed a \emph{root} node, corresponding to the information available at the short-term operational planning decision making point, while the rightmost nodes are termed \emph{leaf} nodes. The \emph{branches} of the scenario tree represent possible transitions between successive \emph{stages} (in the context of the problem, the short-term operational planning decision making point and the real-time intervals within the operational planning horizon). 

Each \emph{path} from the root node to a leaf node defines a unique scenario, that is a possible sequence of random variables $\xi_{1,\dots,T}$, leading to as many scenarios as leaf nodes.  The probability of arriving at any particular node in the tree can be expressed as the product of the conditional probabilities of all the transitions leading to the node in question. In this way, the probability of any unique scenario can also be expressed as the product of the conditional probabilities while following the complete path from the root node to the respective leaf.


It is important to finally notice that  paths are common up to a stage, representing the gradual realization of the exogenous random process. Taking for example the 4 uppermost leaf nodes, we notice that the respective scenarios are indeed common up to $t=1$. This is consistent with the fact that, at this point in time, uncertainty concerning $t=2,3$ remains yet to be resolved. Likewise, the scenarios corresponding to the uppermost 2 nodes would be common for $t=1,2$.

In the remainder of this chapter, we shall use:

\begin{mydescription}{$\hat{S}$}
\item[${S^{\prime}}$]{to denote a finite scenario set approximating the space $S$;}
\item[$\xi_t^{s}$]{to denote the value of random variable $\xi_t$ under scenario $s \in S^{\prime}$; }
\item[$\pi_{s}$]{to denote the probability of $s \in {S}^{\prime}$, with $\sum_{s \in S^{\prime}}=1$.}
\end{mydescription}





\section{Assessment and its possible approximations}
\label{sec:ass}

This section discusses the assessment sub-part of the short-term operational planning reliability management problem. We consider a fixed short-term operational planning decision $\bar{u}_P \in \mathcal{U}_P$  (which may be given \textit{a priori} or void) and focus on analyzing it's implied consequences in light of the possible  realizations $\xi_{1,..T} \in \subset S$. In particular, we frame the evaluation of:



\begin{enumerate}[{[A]}]
\item{\underline{The probability of achieving acceptable system performance.} \medskip \\
From the operational planning perspective,we interpret acceptable system performance as the existence of a feasible solution to the RT-RMAC instances within the concerned horizon. Given $\bar{u}_p$ and the possible realizations of  $\xi_{1,..T} \in \subset S$, the scope is to determine the probability that decision $\bar{u}_p$  renders the RT-RMAC instances within the planning horizon achievable, as in,

\begin{flalign}
\mathbb{P}_{xi_{1,\dots,T} \in S  }\{\delta^{\star}_{RT}(\bar{u}_p,\xi_{t}) = 0 \} = \mathbb{E}_{\xi_{1,\dots,T} \in S}\left\{\mathbf{1}_{\delta_{RT}^{\star}(\bar{u}_p,\xi_{t})  \le 0 }  \right\},&& \label{delta.chance}
\end{flalign}

where we use the notation $[\delta_{RT}^{\star}(\bar{u}_p,\xi_t) = 0]$ to indicate a feasible RT-RMAC. 


%\color{blue}{Reliability Indicator}


}

\item{\underline{The future costs induced by decision $\bar{u}_P$.}\medskip
\\ Here, we seek to quantify, for all real-time problem instances within the horizon  $ t \in [1,T] $, both,

\begin{mydescription}{$W_{RT}\left(\bar{u}_p,u_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right)$}
\item[$W_{RT}\left(\bar{u}_p,u_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right)$:]{the attainable objective function of the RT-RMAC, and,} 
\item[$\delta_{RT}^{\star}(\bar{u}_p,\xi_{t})  $:]{the implied consequences in case the RT-RMAC is not-achievable.} 
\end{mydescription} 

Aggregating these quantities over time and, subject to the uncertainty $\xi_{1,\dots,T} \in S$, we formulate the expectation of future costs implied by any given $\bar{u}_p$, as,  


\begin{flalign}
&\mathbb{E}_{\xi_{1,\dots,T} \in {S}}\left\{ \sum_{t =1}^{T} \left[W_{RT}\left(\bar{u}_p,u^{\star}_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right)  +  \delta_{RT}^{\star}(\bar{u}_p,\xi_{t})  \right] \right\}.& \label{exp.obj}
\end{flalign}

%\color{blue}{Risk indicator}

}

\end{enumerate}


\subsection{Possible Approximations}

For ease of readability, we begin by recalling that, at any $t \in [1,T]$ and given $(\bar{u}_P)$,  real-time reliability management decisions would be,


\begin{flalign}
u^{\star}_{RT}({\xi}_t) \in  \argmin_{u_{RT}({\xi}_t)} &W_{RT}\left(\textcolor{blue}{\bar{u}_p},u_{RT}({\xi}_t), \mathcal{N}_c({\xi}_t)\right) & \label{as.RT.obj.1}\\
&s.t.&\nonumber\\
&u_{RT}(\xi_t) \in \mathcal{U}_{RT}(\textcolor{blue}{\bar{u}_p},\textcolor{blue}{u_{RT}(\xi_{[1,t-1]})},{\xi}_t)  & \label{as.set.RT.1} \\
&\mathbb{P}_{c \in \mathcal{N}_c ({\xi}_t) }  \left \{h\left(\textcolor{blue}{\bar{u}_p},,\xi_t,u_{RT}({\xi}_t)\right)\le  0 \right \}   \ge (1-\varepsilon_{RT}),& \label{as.RT.chance.1}
\end{flalign}
\textbf{while $\mathcal{N}_c({\xi}_t) \subseteq \mathcal{N}(\bar{\xi}_t):$}
\begin{enumerate}[(i.)]
\item  {achieving the RT-RMAC -- \textcolor{darkgreen}{if possible},
\begin{flalign}
& \sum_{c \notin\mathcal{N}_c({\xi}_t)} \pi_{c}({\xi}_t) \cdot c_{R}\left(\textcolor{blue}{\bar{u}_p},{\xi}_t,u^{\star}_{RT}({\xi}_t), c \right) \textcolor{darkgreen}{\le} \Delta{{E}_{RT}},  &\label{as.RT.risk.1}
\end{flalign}
}
\item  {according to the respective relaxation principle -- \textcolor{red}{if not},
\begin{flalign}
& \sum_{c \notin\mathcal{N}_c({\xi}_t)} \pi_{c}({\xi}_t) \cdot c_{R}\left(\textcolor{blue}{\bar{u}_p},{\xi}_t,u^{\star}_{RT}({\xi}_t), c \right)\textcolor{red}{ \not\le }\Delta{{E}_{RT}}.  &\label{as.RT.risk.2}
\end{flalign}}
\end{enumerate}


In \eqref{as.RT.obj.1} -- \eqref{as.RT.risk.2} we use the blue color to highlight the dependence of any RT-RMAC instance on the planning decision under assessment ${\bar{u}_p}$ as well as the on precedent real-time reliability management decisions ${u_{RT}(\xi_{[1,t-1]})}$.  
Notice that as per the latter, both assessment questions [A] and [B] above can only be posed over a sequence of realizations spanning the operational planning horizon $\xi_{1,\dots,T}$.

In light of this feature, we propose to investigate approximate evaluations of  \eqref{delta.chance} and  \eqref{exp.obj} while sampling scenarios\footnote{A brief discussion on sampling techniques is presented on the following chapters of this document.} within the operational planning horizon, \textit{i.e.} sequences of realizations $\xi_{1,\dots,T}$. Evidently, a sequence of realizations forming a particular scenario should be revealed 
in a progressive manner so that the assessment concerning any specific real-time interval $t$ only considers the known realizations ${\xi}_{[t-1]}$ up to this point in time.

We conclude by discussing the atomic variant of the problem, \textit{i.e.} the assessment concerning a single real-time instance  $\bar{\xi}_t$ within a sample $\bar{\xi}_{1,\dots,T} \in S$.  As per \eqref{as.RT.obj.1} -- \eqref{as.RT.risk.1}, a feasible real-time instance should have a solution implying negligible residual risk. In an opposite case, a relaxation will inevitably result in solving \eqref{as.RT.obj.1} -- \eqref{as.RT.chance.1} for a subset of events not meeting condition \eqref{as.RT.risk.1}, \textit{i.e.} for a subset of events implying non-negligible residual risk\footnote{For  example, as per the N-1 criterion, the system operation will not be secured against all the single outages if it is not possible to do so. This would imply the non-negligible risk associated to the occurrence of any unsecured single outage.}. To quantify such non-negligible risk, we propose the following function,
\begin{flalign}
&\delta_{RT}^{\star}(\bar{u}_p,\xi_{t})  =\max\left\{0;\sum_{c \notin\mathcal{N}_c(\xi_t)} \pi_{c}(\xi_t) \cdot c_{R}\left(\bar{u}_p,\xi_t,u^{\star}_{RT}(\xi_t), c\right) - \Delta{{E}_{RT}}\right\}.  & \label{as.con.inf.1}
\end{flalign}

From \eqref{as.con.inf.1}, function $\delta_{RT}^{\star}(\bar{u}_p,\xi_{t}) $  would only take a positive value in the event that the residual risk implied by sub-set $\mathcal{N}_c(\xi_t) \subseteq \mathcal{N}(\xi_t)$ is greater than the respective accuracy limit. Moreover, in any such case, function  $\delta_{RT}^{\star}(\bar{u}_p,\xi_{t})   $ would only measure the extent to which the limit has been exceeded. In other words, this function  essentially measures the implied consequences of relaxing the RT-RMAC, while maintaining the premise that potential consequences up to $\Delta E_{RT}$ should be regarded as negligible. We can thus indeed use the following condition to express a feasible RT-RMAC instance,
\begin{flalign}
&\delta^{\star}_{RT}(\bar{u}_p,\xi_{t}) =0. & \label{feas.cond}
\end{flalign}
The evaluation of \eqref{as.con.inf.1} does not increase the computational complexity of the problem with respect to the formulations already introduced in  Chapter~\ref{chp:realtime} . Rather, the evaluation of \eqref{as.con.inf.1} is a by-product of computing the residual risk implied by any chosen sub-set $\mathcal{N}_c(\xi_t) \subseteq \mathcal{N}(\xi_t)$. Moreover, the possible  ways of approximating such residual risk, discussed in Chapter~\ref{chp:realtime} , respectively result in approximations of the consequences of not achieving the RT-RMAC.

Here, we must underline the potential to exploit the pessimistic approximation to the residual risk quantification to formulate a conservative feasibility assessment sub-problem of reduced complexity. First, recall that the pessimistic approximation involves a conservative upper bound instead of an exact computation of the criticality of service interruption to express a worst-case residual risk value, as in, 

\begin{flalign}
& \sum_{c \notin\mathcal{N}_c(\xi_t)} \pi_{c}(\xi_t) \cdot c_{R}\left(u_p,\xi_t,u^{\star}_{RT}(\xi_t), c \right) \le c_{R}^{max}(\bar{u}_P;\bar{\xi}_t)  \sum_{c \notin\mathcal{N}_c(\xi_t)} \pi_{c}(\xi_t)  \le \Delta E_{RT}. &\label{pess.2}
\end{flalign}

where, 

\begin{mydescription}{$cr_{RT}^{max}({u}_P;{\xi}_t)$)}
\item[$c_{R}^{max}({u}_P;{\xi}_t)$] denotes the maximum criticality value as a function of short-term operational planning decisions as well as uncertainty realizations\footnote{Notice that here we express the upper bound of the criticality value as a function of operational planning decisions ${u}_P$ and uncertainty realization $\xi_t$ to acknowledge that, from the planning perspective, relevant decisions (\textit{e.g.,} the pre-notification of a risk in the electricity supply) as well as random factors (\textit{e.g.,} the weather condition) may possibly influence this maximum criticality value.}.
\end{mydescription}

The rightmost inequality in \eqref{pess.2} defines  (possibly several) sub-sets that should, in the worst-case, be considered of negligible residual risk. We propose to use the smallest such  sub-set as a first step in verifying whether or not $(\bar{u}_p,\bar{\xi}_t)$ jointly result in  a feasible RT-RMAC. Notice that given $(\bar{u}_p,\bar{\xi}_t)$ and the smallest sub-set derived by the pessimistic approximation, the feasibility assessment problem reduces to verifying the existence of a solution to satisfy chance constraint \eqref{as.RT.chance.1}, and can be approximated using a parameter of sufficiently large value $(M)$ as in,  
\begin{flalign}
&\delta_{RT}^{\star}(\bar{u}_p,\xi_{t})   = 0,&\\
\intertext{\textbf{where,}}
 &[u^{\star}_{RT}(\xi_t);\delta^{\star}_{RT}(u_p,\xi_{t})] \in  \argmin_{u_{RT}(\xi_t), \delta_{RT}(u_p,\xi_{t})}[ W_{RT}\left(u_p,u_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) + \delta_{RT}(u_p,\xi_{t}) \cdot M]& \label{as41}\\
&s.t.&\nonumber\\
&u_{RT}(\xi_t) \in \mathcal{U}_{RT}(u_p,u_{RT}(\xi_{[1,t-1]}),\xi_t)    & \label{as42}\\
&\mathbb{P}_{c \in \mathcal{N}_c (\xi_t) }  \left \{h\left(u_p,\xi_t,u_{RT}(\xi_t)\right)\le  0  \right \} \ge (1-\varepsilon_{RT})- \delta_{RT}(u_p,\xi_{t}),&  \label{DA.43}\\
&\delta_{RT}(u_p,\xi_{t})\ge 0.&\label{as44}
\end{flalign}

Validating  \eqref{feas.cond} for the smallest sub-set derived from the pessimistic approximation is a \emph{sufficient} but not \emph{necessary} condition for the feasibility of the RT-RMAC. In other words, finding such a solution suffices to warrant the feasibility of the RT-RMAC while not finding such a solution does not imply that the RT-RMAC is indeed infeasible. We may thus consider the use of the pessimistic approximation to derive conservative guarantees of the feasibility of the RT-RMAC.

\section{Decision making and its possible approximations}
\label{sec:dec}

Using the introduced notation, we begin by stating the general formulation of the short-term operational planning problem as, 



\begin{flalign}
\min_{u_p }& \left\{ 
 C_P(u_p) +\mathbb{E}_{\xi_{1,\dots,T} \in {S}}\left\{ \sum_{t =1}^{T}\left[W_{RT}\left(u_p,u^{\star}_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) + \delta_{RT}^{\star}(u_p,\xi_{t})    \right]\right\} \right \} & \label{DA.01} \\
s.t.&&\nonumber\\
&u_p \in{U}_p & \label{DA.02} \\
&\forall \xi_{1,\dots,T} \in {S}:&\nonumber\\
&\mathcal{N}_c({\xi_t}) \subseteq \mathcal{N}({\xi_t})  &\label{DA.03} \\
&\delta_{RT}^{\star}(u_p,\xi_{t})    \ge  \sum_{c \notin\mathcal{N}_c(\mathbf{s}_t)} \pi_{c}(\xi_t) \cdot c_{R}\left(u_p,\xi_t,u^{\star}_{RT}(\xi_t), c\right)  - \Delta{{E}_{RT}} & \label{DA.04} \\
&\delta_{RT}^{\star}(u_p,\xi_{t})       \ge 0 & \label{DA.05} \\
 &u^{\star}_{RT}(\xi_t) \in  \argmin_{u_{RT}(\xi_t)} W_{RT}\left(u_p,u_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) & \label{DA.06}\\
&s.t.&\nonumber\\
&u_{RT}(\xi_t) \in \mathcal{U}_{RT}(u_p,u_{RT}(\xi_{[1,t-1]}),\xi_t)    & \label{DA.09}\\
&\mathbb{P}_{c \in \mathcal{N}_c (\xi_t) }  \left \{h\left(u_p,\xi_t,u_{RT}(\xi_t)\right)\le  0 \right \} \ge (1-\varepsilon_{RT}).&  \label{DA.08}
\end{flalign}



%-----
\begin{figure}
\begin{framed}
\begin{center}
\begin{tabular}{c| ccc}
\multicolumn{4}{c}{}\\
 & \multicolumn{3}{c}{\emph{\textcolor{shadecolor}{\textbf{Select  \&  apply}}}  $\color{shadecolor}{ 	u^{\star}_{RT}(\xi_t) \in \mathcal{U}_{RT}(u_p,\xi_t)  }$}\\
$
\begin{array}{c}
\textbf{\emph{Select  \&  apply}} 	\\
u_p \in \mathcal{U}_p\\
\downarrow\\
\bullet \\
\\
\\
\\
\end{array}
$
%---------------
&
%--------------
$\begin{array}{c}
\\
\nearrow\\
\xi_1\rightarrow\\
\searrow\\
\\
\end{array}
 \color{shadecolor}{
\begin{array}{c}
\downarrow\\
\bullet \\
.\\
 .\\
.\\
.\\
\bullet \\
\end{array}} 
$
%---------------
&
%--------------
$\begin{array}{c}
\\
\nearrow\\
\xi_{1,\dots,t}\rightarrow\\
\searrow\\
\\
\end{array}
\color{shadecolor}{
\begin{array}{c}
\downarrow\\
\bullet  \\
.\\
 .\\
.\\
.\\
\bullet \\
\end{array}  
}$
%---------------
&
%--------------
$
\begin{array}{c}
\\
\nearrow\\
\xi_{1, \dots, T} \rightarrow\\
\searrow\\
\\
\end{array}

\color{shadecolor}{
\begin{array}{c}
\downarrow\\
\bullet  \\
.\\
 .\\
.\\
.\\
\bullet \\
\end{array} }
$

\\
\dotfill&\multicolumn{3}{c}{\textcolor{shadecolor}{ \dotfill}}\\
$\downarrow$&\multicolumn{3}{c}{\textcolor{shadecolor}{$ \downarrow \forall t \in [1,T] \downarrow$}}\\
\dotfill&\multicolumn{3}{c}{\textcolor{shadecolor}{ \dotfill}}\\
{$C_p(u_p)$}&\multicolumn{3}{c}{$\textcolor{shadecolor}{ W_{RT}\left(u_p,u^{\star}_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) + \delta_{RT}^{\star}(u_p,\xi_{t})    }$}\\
\end{tabular}\\

\end{center}

\end{framed}

\caption{Short-term operational planning reliabilty management}
\label{fig:DAmgmt}
\end{figure}
%--------------------------------------------------------------------------




The objective of the short-term operational planning reliability management problem (Fig. \ref{fig:DAmgmt}) is the minimization of all relevant socio-economic costs \eqref{DA.01}. We notice that the second term of \eqref{DA.01} expresses the implied consequences of any short-term operational planning decision on real-time reliability management, as an expectation over the sequence of random variables ($\xi_{1,\dots,T}$). In other words, the second term of \eqref{DA.01} expresses risk as perceived in the short-term operational planning context.

Expression \eqref{DA.02} imposes short-term operational planning decisions to be chosen within the respective admissible set. Expressions \eqref{DA.03} -- \eqref{DA.08} relate to the effect of short-term operational planning decisions on real-time reliability management.

 Particularly, \eqref{DA.03} formalizes the consideration of a sub-set of contingency events, as per the respective RT-RMAC. Since the consequences of any contingency event  may depend on  short-term operational planning decisions, any sub-set $\mathcal{N}_c(\xi_t)$  would implicitly depend on short-term operational planning decisions as well. We underline that the choice of any sub-set $\mathcal{N}_c(\xi_t)$ essentially depends on  whether or not the  RT-RMAC can be achieved or must relaxed.  

More specifically, for any operational planning decision ($u_p$) and sub-set $\mathcal{N}_c(\xi_t)$,  the corresponding real-time reliability management decisions $u^{\star}_{RT}(\xi_t)$ would be defined as in \eqref{DA.06} -- \eqref{DA.08}. In the event that such decisions indeed achieve the RT-RMAC, there will be no consequences of relaxation (since no relaxation is necessary). Constraint  \eqref{DA.05} is thus used to restrict the consequences of relaxing the RT-RMAC to non-zero values. This constraint will be active in any case the RT-RMAC is achievable. In any opposite case, the consequences of relaxing the RT-RMAC would take positive values as in \eqref{DA.04}.


Recalling that operational planning decisions influence the potential to achieve the RT-RMAC, formulation  \eqref{DA.01} -- \eqref{DA.08} seeks for a tradeoff between the costs of operational planning actions and the expected costs of achieving the RT-RMAC as well as the implied consequences of not doing so. In other words, formulation \eqref{DA.01} -- \eqref{DA.08} seeks for operational planning decisions making the RT-RMAC feasible only under the condition that doing so leads to the minimization of all relevant socio-economic costs in the short-term operational planning context. 



\subsection{Short-term operational planning RMAC}

On the basis of \eqref{DA.01} -- \eqref{DA.08}, we can introduce the short-term operational planning RMAC (OP-RMAC). We propose to focus on mitigate the risk implied by the uncertainty $\xi_{1,\dots,T} \in S$  (\textit{i.e.} the second terms of \eqref{DA.01}) by:



\begin{enumerate}[{[A.]}]
\item{\underline{Forming a (dynamic) subset of realizations $S_c \subset S$}\\

The scope is to identify and neglect from \eqref{DA.01} -- \eqref{DA.08}  a sub-space of the possible realizations $\xi_{1,..T} \notin S_c \subset S$, in order to reduce uncertainty to a manageable size.   We shall again rely on the principle of neglecting possible realizations of negligible residual risk, as in lower than a pre-specified accuracy limit. Denoting the latter as $\Delta E_{OP}$, we state the resulting condition as, 
\begin{flalign}
&\mathbb{E}_{\xi_{1,\dots,T} \notin {S}_c}\left\{ \sum_{t =1}^{T}\left[W_{RT}\left(u_p,u^{\star}_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) + \delta_{RT}^{\star}(u_p,\xi_{t})    \right]\right\} \le \Delta E_{OP},&\label{DA.19}\\
&\color{shadecolor}\left\{\begin{array}{l}
\mathcal{N}_c({\xi_t}) \subseteq \mathcal{N}({\xi_t})  \\
\delta_{RT}^{\star}(u_p,\xi_{t})    \ge  \sum_{c \notin\mathcal{N}_c(\mathbf{s}_t)} \pi_{c}(\xi_t) \cdot c_{R}\left(u_p,\xi_t,u^{\star}_{RT}(\xi_t), c\right)  - \Delta{{E}_{RT}} \\
\delta_{RT}^{\star}(u_p,\xi_{t})       \ge 0 \\
 u^{\star}_{RT}(\xi_t) \in  \argmin_{u_{RT}(\xi_t)} W_{RT}\left(u_p,u_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) \\
 s.t.\\
 u_{RT}(\xi_t) \in \mathcal{U}_{RT}(u_p,u_{RT}(\xi_{[1,t-1]}),\xi_t)    \\
\mathbb{P}_{c \in \mathcal{N}_c (\xi_t) }  \left \{h\left(u_p,\xi_t,u_{RT}(\xi_t)\right)\le  0 \right \} \ge (1-\varepsilon_{RT})
\end{array}\right\},&\\
&\color{shadecolor}\forall \xi_{1,\dots,T} \notin S_c. &\nonumber 
\end{flalign}

Notice that this is an extension of the discarding principle already introduced in Chapter~\ref{chp:realtime}  to identify contingency subsets of negligible residual risk. We briefly re-state that this principle allows to dynamically reduce the uncertainty space while  probabilities and/or potentially consequences are variable.


}

\item{\underline{Ensuring acceptable performance \textit{vs} $\xi_{1,\dots,T} \in S_c$}\\

To complement the discarding principle introduced above, we concentrate on the sub-space  $S_c \subset S$, within which short-term operational planning decisions should be considered to mitigate the potential consequences. Within this sub-space, we propose to consider  an explicit requirement on the feasibility of the RT-RMAC, as in, 


\begin{flalign}
&\delta^{\star}_{RT}(u_p,\xi_{t}) \le 0 \quad \forall \xi_{1,\dots,T}\in S_c,  & \label{zero.delta}\\
&\color{shadecolor}\left\{\begin{array}{l}
\mathcal{N}_c({\xi_t}) \subseteq \mathcal{N}({\xi_t})  \\
\delta_{RT}^{\star}(u_p,\xi_{t})    \ge  \sum_{c \notin\mathcal{N}_c(\mathbf{s}_t)} \pi_{c}(\xi_t) \cdot c_{R}\left(u_p,\xi_t,u^{\star}_{RT}(\xi_t), c\right)  - \Delta{{E}_{RT}} \\
\delta_{RT}^{\star}(u_p,\xi_{t})       \ge 0 \\
 u^{\star}_{RT}(\xi_t) \in  \argmin_{u_{RT}(\xi_t)} W_{RT}\left(u_p,u_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) \\
 s.t.\\
 u_{RT}(\xi_t) \in \mathcal{U}_{RT}(u_p,u_{RT}(\xi_{[1,t-1]}),\xi_t)    \\
\mathbb{P}_{c \in \mathcal{N}_c (\xi_t) }  \left \{h\left(u_p,\xi_t,u_{RT}(\xi_t)\right)\le  0 \right \} \ge (1-\varepsilon_{RT})
\end{array}\right\},&\label{RTprx1}\\
&\color{shadecolor}\forall \xi_{1,\dots,T}\in S_c.& \nonumber
\end{flalign}

%Under \eqref{zero.delta} -- \eqref{RTprx1}, it suffices to express the implied consequences of any short-term operational planning decision $u_p \in \mathcal{U}_p$ within $S_c \subset S$ as,
%\begin{flalign}
%\mathbb{E}_{\xi_{1,\dots,T} \in {S}_c}\left\{ \sum_{t =1}^{T}W_{RT}\left(u_p,u^{\star}_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) \right\}.&& 
%\end{flalign}

}
\end{enumerate}


%Here, we should underline that, as per [A.]



Taking both [A.] and [B.] above into consideration, we can state the OP-RMAC as, 

\begin{framed}
\begin{flalign}
&\min_{u_p }\left[
 C_P(u_p) +\mathbb{E}_{\xi_{1,\dots,T} \in {S}_c}\left\{ \sum_{t =1}^{T}W_{RT}\left(u_p,u^{\star}_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) \right\}  \right] & \label{DA.41} \\
\intertext{s.t.}
&u_p \in{U}_p & \label{DA.42} \\
&\delta^{\star}_{RT}(u_p,\xi_{t}) \le 0,  \forall \xi_{1,\dots,T} \in {S}_c,&\label{zero.delta2}\\
\intertext{while,}
&S_c\subset S: \mathbb{E}_{\xi_{1,\dots,T} \notin {S}_c}\left\{ \sum_{t =1}^{T}\left[W_{RT}\left(u_p,u^{\star}_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) + \delta_{RT}^{\star}(u_p,\xi_{t})    \right]\right\} \le \Delta E_{OP},& \label{DA.ResR} \\
&\color{shadecolor}\left\{\begin{array}{l}
\mathcal{N}_c({\xi_t}) \subseteq \mathcal{N}({\xi_t})  \\
\delta_{RT}^{\star}(u_p,\xi_{t})    \ge  \sum_{c \notin\mathcal{N}_c(\mathbf{s}_t)} \pi_{c}(\xi_t)  c_{R} \left(u_p,\xi_t,u^{\star}_{RT}(\xi_t), c\right)  - \Delta{{E}_{RT}} \\
\delta_{RT}^{\star}(u_p,\xi_{t})       \ge 0 \\
 u^{\star}_{RT}(\xi_t) \in  \argmin_{u_{RT}(\xi_t)} W_{RT}\left(u_p,u_{RT}(\xi_t), \mathcal{N}_c(\xi_t)\right) \\
 s.t.\\
 u_{RT}(\xi_t) \in \mathcal{U}_{RT}(u_p,u_{RT}(\xi_{[1,t-1]}),\xi_t)    \\
\mathbb{P}_{c \in \mathcal{N}_c (\xi_t) }  \left \{h\left(u_p,\xi_t,u_{RT}(\xi_t)\right)\le  0 \right \} \ge (1-\varepsilon_{RT})
\end{array}\right\}, \label{DA.49}\\
&\color{shadecolor}\forall \xi_{1,\dots,T} \in S .& \nonumber
\end{flalign}
\end{framed}




We should clarify that,  under \eqref{zero.delta2},  it suffices to express the implied consequences of any short-term operational planning decision $u_p \in \mathcal{U}_p$ within $S_c \subset S$ as in the second term of  \eqref{DA.41}. Moreover, note that the set of expressions \eqref{DA.49} groups the model of the real-time decision making process, as per the respective RT-RMAC. Even though not explicitly shown,  models of different complexity (\textit{i.e.}, different proxies) may be used for the solution of \eqref{DA.41} --\eqref{zero.delta2} and the evaluation of condition \eqref{DA.ResR}.




\subsection{Possible approximations}

We acknowledge here that the solution of \eqref{DA.41} -- \eqref{DA.49} is far from trivial. Let us briefly underline the following challenges:

\begin{itemize}
\item[{$\blacktriangleright$}]{The general case of a continuously distributed random variable $(\xi_t)$ implies an infinite number of possible realizations for the single respective real-time interval. Evidently, this also implies an infinite number of  anticipated real-time decisions $u_{RT}^{\star}(\xi_t)$ for any single $t \in [1,T]$. }
\item[{$\blacktriangleright$}]{As already introduced, the set of candidate real-time  decisions at any $t \in [1,T]$ may depend on precedent real-time reliability management decisions $u_{RT}(\xi_{[t-1]})$. Hence, constraint \eqref{zero.delta2}, should be jointly satisfied by all real-time decisions corresponding to a unique sequence of realizations $\xi_{1,\dots,T}$. Moreover, at any intermediate step $t < T$ the aforementioned real-time decisions should be \emph{non-anticipative}, \textit{i.e.} agnostic on the future realizations $\xi_{t+1,\dots,T}$.}
\end{itemize}

 %

The development of appropriate approximation remains on-going work within GARPUR Task~2.3. Be that as it may, we discuss here approximations of relevance.

To particularly tackle the issues above, we propose to begin by exploiting the scenario tree approximation introduced in section \ref{sec:unct} and re-cast \eqref{DA.41} -- \eqref{DA.49} over a discrete set of potential sequences of realizations $S_c^{\prime} \subset S$. We underline here the potential utility of this approach in complementarity to the discarding principle \eqref{DA.ResR}. Indeed, combining these two aspects it becomes relevant to investigate (i) identifying a solution to \eqref{DA.41} -- \eqref{zero.delta2} while \eqref{DA.49} over a discrete set of realizations $S_c^{\prime}= \{\xi_{1,\dots,T}^{1};\dots,\xi_{1,\dots,T}^{|S^{\prime}|} \}$, and, (ii) evaluating the implied residual risk \eqref{DA.ResR} over $S\setminus S_c^{\prime}$.

Finally, we should also consider the resulting problem \eqref{DA.41} -- \eqref{zero.delta2} while \eqref{DA.49} over a discrete set of realizations $S_c^{\prime}= \{\xi_{1,\dots,T}^{1};\dots,\xi_{1,\dots,T}^{|S^{\prime}|} \}$. As a possible way to tackle the complexity of this problem, we propose to investigate scenario decomposition techniques, namely the \emph{progressive hedging algorithm}. Referring the reader to \cite{Rockafellar} for a detailed presentation of this algorithm, we briefly explain that the approach relies on solving separately the sub-problems corresponding to any specific scenario $s \in \mathcal{S}^{\prime}$ while iteratively converging to non-anticipative decisions.











\color{black}



==> 221/IEEEfull.tex <==

IEEEfull.bib
V1.13 (2008/09/30)
Copyright (c) 2002-2008 by Michael Shell
See: http://www.michaelshell.org/
for current contact information.

BibTeX bibliography string definitions of the FULL titles of
IEEE journals and magazines and online publications.

This file is designed for bibliography styles that require 
full-length titles and is not for use in bibliographies that
abbreviate titles.

Support sites:
http://www.michaelshell.org/tex/ieeetran/
http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/
and/or
http://www.ieee.org/

Special thanks to Laura Hyslop and ken Rawson of IEEE for their help
in obtaining the information needed to compile this file. Also,
Volker Kuhlmann and Moritz Borgmann kindly provided some corrections
and additions.

*************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEabrv.bib, IEEEfull.bib, IEEEexample.bib,
                   IEEEtran.bst, IEEEtranS.bst, IEEEtranSA.bst,
                   IEEEtranN.bst, IEEEtranSN.bst, IEEEtran_bst_HOWTO.pdf
*************************************************************************


USAGE:

\bibliographystyle{mybstfile}
\bibliography{IEEEfull,mybibfile}

where the IEEE titles in the .bib database entries use the strings
defined here. e.g.,


   journal = IEEE_J_AC,


to yield "{IEEE} Transactions on Automatic Control"


WARNING: IEEE uses abbreviated journal titles in their bibliographies!
Because this file provides the full titles, you should NOT use this file
for work that is to be submitted to the IEEE.

For IEEE work, you should use the abbreviated titles provided in the
companion file, IEEEabrv.bib.


** NOTES **

 1. Journals have been grouped according to subject in order to make it
    easier to locate and extract the definitions for related journals - 
    as most works use references that are confined to a single topic.
    Magazines are listed in straight alphabetical order.

 2. String names are closely based on IEEE's own internal acronyms.

 3. Older, out-of-print IEEE titles are included (but not including titles
    dating prior to IEEE's formation from the IRE and AIEE in 1963).






IEEE Journals 



aerospace and military
@STRING{IEEE_J_AES        = "{IEEE} Transactions on Aerospace and Electronic Systems"}
@STRING{IEEE_J_ANE        = "{IEEE} Transactions on Aerospace and Navigational Electronics"}
@STRING{IEEE_J_ANNE       = "{IEEE} Transactions on Aeronautical and Navigational Electronics"}
@STRING{IEEE_J_AS         = "{IEEE} Transactions on Aerospace"}
@STRING{IEEE_J_AIRE       = "{IEEE} Transactions on Airborne Electronics"}
@STRING{IEEE_J_MIL        = "{IEEE} Transactions on Military Electronics"}



autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Transactions on Intelligent Transportation Systems"}
@STRING{IEEE_J_VT         = "{IEEE} Transactions on Vehicular Technology"}
@STRING{IEEE_J_VC         = "{IEEE} Transactions on Vehicular Communications"}



circuits, signals, systems, audio and controls
@STRING{IEEE_J_SPL        = "{IEEE} Signal Processing Letters"}
@STRING{IEEE_J_ASSP       = "{IEEE} Transactions on Acoustics, Speech, and Signal Processing"}
@STRING{IEEE_J_AU         = "{IEEE} Transactions on Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Transactions on Audio and Electroacoustics"}
@STRING{IEEE_J_AC         = "{IEEE} Transactions on Automatic Control"}
@STRING{IEEE_J_CAS        = "{IEEE} Transactions on Circuits and Systems"}
@STRING{IEEE_J_CASVT      = "{IEEE} Transactions on Circuits and Systems for Video Technology"}
@STRING{IEEE_J_CASI       = "{IEEE} Transactions on Circuits and Systems---Part {I}: Fundamental Theory and Applications"}
@STRING{IEEE_J_CASII      = "{IEEE} Transactions on Circuits and Systems---Part {II}: Analog and Digital Signal Processing"}
in 2004 CASI and CASII renamed part title to CASI_RP and CASII_EB, respectively.
@STRING{IEEE_J_CASI_RP    = "{IEEE} Transactions on Circuits and Systems---Part {I}: Regular Papers"}
@STRING{IEEE_J_CASII_EB   = "{IEEE} Transactions on Circuits and Systems---Part {II}: Express Briefs"}
@STRING{IEEE_J_CT         = "{IEEE} Transactions on Circuit Theory"}
@STRING{IEEE_J_CST        = "{IEEE} Transactions on Control Systems Technology"}
@STRING{IEEE_J_SP         = "{IEEE} Transactions on Signal Processing"}
@STRING{IEEE_J_SU         = "{IEEE} Transactions on Sonics and Ultrasonics"}
@STRING{IEEE_J_SAP        = "{IEEE} Transactions on Speech and Audio Processing"}
@STRING{IEEE_J_STSP       = "{IEEE} Journal of Selected Topics in Signal Processing"}
@STRING{IEEE_J_SYST       = "{IEEE} Systems Journal"}
@STRING{IEEE_J_UE         = "{IEEE} Transactions on Ultrasonics Engineering"}
@STRING{IEEE_J_UFFC       = "{IEEE} Transactions on Ultrasonics, Ferroelectrics, and Frequency Control"}



communications
@STRING{IEEE_J_COML       = "{IEEE} Communications Letters"}
@STRING{IEEE_J_JSAC       = "{IEEE} Journal on Selected Areas in Communications"}
@STRING{IEEE_J_COM        = "{IEEE} Transactions on Communications"}
@STRING{IEEE_J_COMT       = "{IEEE} Transactions on Communication Technology"}
@STRING{IEEE_J_WCOM       = "{IEEE} Transactions on Wireless Communications"}



components, packaging and manufacturing
@STRING{IEEE_J_ADVP       = "{IEEE} Transactions on Advanced Packaging"}
@STRING{IEEE_J_CHMT       = "{IEEE} Transactions on Components, Hybrids and Manufacturing Technology"}
@STRING{IEEE_J_CPMTA      = "{IEEE} Transactions on Components, Packaging and Manufacturing Technology---Part {A}"}
@STRING{IEEE_J_CPMTB      = "{IEEE} Transactions on Components, Packaging and Manufacturing Technology---Part {B}: Advanced Packaging"}
@STRING{IEEE_J_CPMTC      = "{IEEE} Transactions on Components, Packaging and Manufacturing Technology---Part {C}: Manufacturing"}
@STRING{IEEE_J_CAPT       = "{IEEE} Transactions on Components and Packaging Technology"}
@STRING{IEEE_J_CAPTS      = "{IEEE} Transactions on Components and Packaging Technologies"}
@STRING{IEEE_J_CPART      = "{IEEE} Transactions on Component Parts"}
@STRING{IEEE_J_EPM        = "{IEEE} Transactions on Electronics Packaging Manufacturing"}
@STRING{IEEE_J_MFT        = "{IEEE} Transactions on Manufacturing Technology"}
@STRING{IEEE_J_PHP        = "{IEEE} Transactions on Parts, Hybrids and Packaging"}
@STRING{IEEE_J_PMP        = "{IEEE} Transactions on Parts, Materials and Packaging"}



CAD
@STRING{IEEE_J_TCAD       = "{IEEE} Journal on Technology in Computer Aided Design"}
@STRING{IEEE_J_CAD        = "{IEEE} Transactions on Computer-Aided Design of Integrated Circuits and Systems"}



coding, data, information, knowledge
@STRING{IEEE_J_IT         = "{IEEE} Transactions on Information Theory"}
@STRING{IEEE_J_KDE        = "{IEEE} Transactions on Knowledge and Data Engineering"}



computers, computation, networking and software
@STRING{IEEE_J_C          = "{IEEE} Transactions on Computers"}
@STRING{IEEE_J_CAL        = "{IEEE} Computer Architecture Letters"}
@STRING{IEEE_J_DSC        = "{IEEE} Transactions on Dependable and Secure Computing"}
@STRING{IEEE_J_ECOMP      = "{IEEE} Transactions on Electronic Computers"}
@STRING{IEEE_J_EVC        = "{IEEE} Transactions on Evolutionary Computation"}
@STRING{IEEE_J_FUZZ       = "{IEEE} Transactions on Fuzzy Systems"}
@STRING{IEEE_J_IFS        = "{IEEE} Transactions on Information Forensics and Security"}
@STRING{IEEE_J_MC         = "{IEEE} Transactions on Mobile Computing"}
@STRING{IEEE_J_NET        = "{IEEE/ACM} Transactions on Networking"}
@STRING{IEEE_J_NN         = "{IEEE} Transactions on Neural Networks"}
@STRING{IEEE_J_NSM        = "{IEEE} Transactions on Network and Service Management"}
@STRING{IEEE_J_PDS        = "{IEEE} Transactions on Parallel and Distributed Systems"}
@STRING{IEEE_J_SC         = "{IEEE} Transactions on Services Computing"}
@STRING{IEEE_J_SE         = "{IEEE} Transactions on Software Engineering"}



computer graphics, imaging, and multimedia
@STRING{IEEE_J_JDT        = "{IEEE/OSA} Journal of Display Technology"}
@STRING{IEEE_J_IP         = "{IEEE} Transactions on Image Processing"}
@STRING{IEEE_J_MM         = "{IEEE} Transactions on Multimedia"}
@STRING{IEEE_J_VCG        = "{IEEE} Transactions on Visualization and Computer Graphics"}



cybernetics, ergonomics, robots, man-machine, and automation
@STRING{IEEE_J_ASE        = "{IEEE} Transactions on Automation Science and Engineering"}
@STRING{IEEE_J_JRA        = "{IEEE} Journal of Robotics and Automation"}
@STRING{IEEE_J_H          = "{IEEE} Transactions on Haptics"}
@STRING{IEEE_J_HFE        = "{IEEE} Transactions on Human Factors in Electronics"}
@STRING{IEEE_J_MMS        = "{IEEE} Transactions on Man-Machine Systems"}
@STRING{IEEE_J_PAMI       = "{IEEE} Transactions on Pattern Analysis and Machine Intelligence"}
in 1989 JRA became RA
in August 2004, RA split into ASE and RO
@STRING{IEEE_J_RA         = "{IEEE} Transactions on Robotics and Automation"}
@STRING{IEEE_J_RO         = "{IEEE} Transactions on Robotics"}
@STRING{IEEE_J_SMC        = "{IEEE} Transactions on Systems, Man, and Cybernetics"}
@STRING{IEEE_J_SMCA       = "{IEEE} Transactions on Systems, Man, and Cybernetics---Part {A}: Systems and Humans"}
@STRING{IEEE_J_SMCB       = "{IEEE} Transactions on Systems, Man, and Cybernetics---Part {B}: Cybernetics"}
@STRING{IEEE_J_SMCC       = "{IEEE} Transactions on Systems, Man, and Cybernetics---Part {C}: Applications and Reviews"}
@STRING{IEEE_J_SSC        = "{IEEE} Transactions on Systems Science and Cybernetics"}



earth, wind, fire and water
@STRING{IEEE_J_GE         = "{IEEE} Transactions on Geoscience Electronics"}
@STRING{IEEE_J_GRS        = "{IEEE} Transactions on Geoscience and Remote Sensing"}
@STRING{IEEE_J_GRSL       = "{IEEE} Geoscience and Remote Sensing Letters"}
@STRING{IEEE_J_OE         = "{IEEE} Journal of Oceanic Engineering"}
@STRING{IEEE_J_STARS      = "{IEEE} Journal of Selected Topics in Applied Earth Observations and Remote Sensing"}



education, engineering, history, IEEE, professional
@STRING{IEEE_J_CJECE      = "Canadian Journal of Electrical and Computer Engineering"}
@STRING{IEEE_J_PROC       = "Proceedings of the {IEEE}"}
@STRING{IEEE_J_EDU        = "{IEEE} Transactions on Education"}
@STRING{IEEE_J_EM         = "{IEEE} Transactions on Engineering Management"}
@STRING{IEEE_J_EWS        = "{IEEE} Transactions on Engineering Writing and Speech"}
@STRING{IEEE_J_LT         = "{IEEE} Transactions on Learning Technologies"}
@STRING{IEEE_J_PC         = "{IEEE} Transactions on Professional Communication"}



electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas and Wireless Propagation Letters"}
@STRING{IEEE_J_MGWL       = "{IEEE} Microwave and Guided Wave Letters"}
@STRING{IEEE_J_MWCL       = "{IEEE} Microwave and Wireless Components Letters"}
@STRING{IEEE_J_AP         = "{IEEE} Transactions on Antennas and Propagation"}
@STRING{IEEE_J_EMC        = "{IEEE} Transactions on Electromagnetic Compatibility"}
@STRING{IEEE_J_MAG        = "{IEEE} Transactions on Magnetics"}
@STRING{IEEE_J_MTT        = "{IEEE} Transactions on Microwave Theory and Techniques"}
@STRING{IEEE_J_RFI        = "{IEEE} Transactions on Radio Frequency Interference"}
@STRING{IEEE_J_TJMJ       = "{IEEE} Translation Journal on Magnetics in Japan"}



energy and power
@STRING{IEEE_J_EC         = "{IEEE} Transactions on Energy Conversion"}
@STRING{IEEE_J_PEL        = "{IEEE} Power Electronics Letters"}
@STRING{IEEE_J_PWRAS      = "{IEEE} Transactions on Power Apparatus and Systems"}
@STRING{IEEE_J_PWRD       = "{IEEE} Transactions on Power Delivery"}
@STRING{IEEE_J_PWRE       = "{IEEE} Transactions on Power Electronics"}
@STRING{IEEE_J_PWRS       = "{IEEE} Transactions on Power Systems"}



industrial, commercial and consumer
@STRING{IEEE_J_APPIND     = "{IEEE} Transactions on Applications and Industry"}
@STRING{IEEE_J_BC         = "{IEEE} Transactions on Broadcasting"}
@STRING{IEEE_J_BCTV       = "{IEEE} Transactions on Broadcast and Television Receivers"}
@STRING{IEEE_J_CE         = "{IEEE} Transactions on Consumer Electronics"}
@STRING{IEEE_J_IE         = "{IEEE} Transactions on Industrial Electronics"}
@STRING{IEEE_J_IECI       = "{IEEE} Transactions on Industrial Electronics and Control Instrumentation"}
@STRING{IEEE_J_IA         = "{IEEE} Transactions on Industry Applications"}
@STRING{IEEE_J_IGA        = "{IEEE} Transactions on Industry and General Applications"}
@STRING{IEEE_J_IINF       = "{IEEE} Transactions on Industrial Informatics"}
@STRING{IEEE_J_PSE        = "{IEEE} Journal of Product Safety Engineering"}



instrumentation and measurement
@STRING{IEEE_J_IM         = "{IEEE} Transactions on Instrumentation and Measurement"}



insulation and materials
@STRING{IEEE_J_JEM        = "{IEEE/TMS} Journal of Electronic Materials"}
@STRING{IEEE_J_DEI        = "{IEEE} Transactions on Dielectrics and Electrical Insulation"}
@STRING{IEEE_J_EI         = "{IEEE} Transactions on Electrical Insulation"}



mechanical
@STRING{IEEE_J_MECH       = "{IEEE/ASME} Transactions on Mechatronics"}
@STRING{IEEE_J_MEMS       = "{IEEE/ASME} Journal of Microelectromechanical Systems"}



medical and biological
@STRING{IEEE_J_BCAS       = "{IEEE} Transactions on Biomedical Circuits and Systems"}
@STRING{IEEE_J_BME        = "{IEEE} Transactions on Biomedical Engineering"}
Note: The B-ME journal later dropped the hyphen and became the BME.
@STRING{IEEE_J_B-ME       = "{IEEE} Transactions on Bio-Medical Engineering"}
@STRING{IEEE_J_BMELC      = "{IEEE} Transactions on Bio-Medical Electronics"}
@STRING{IEEE_J_CBB        = "{IEEE/ACM} Transactions on Computational Biology and Bioinformatics"}
@STRING{IEEE_J_ITBM       = "{IEEE} Transactions on Information Technology in Biomedicine"}
@STRING{IEEE_J_ME         = "{IEEE} Transactions on Medical Electronics"}
@STRING{IEEE_J_MI         = "{IEEE} Transactions on Medical Imaging"}
@STRING{IEEE_J_NB         = "{IEEE} Transactions on NanoBioscience"}
@STRING{IEEE_J_NSRE       = "{IEEE} Transactions on Neural Systems and Rehabilitation Engineering"}
@STRING{IEEE_J_RBME       = "{IEEE} Reviews in Biomedical Engineering"}
@STRING{IEEE_J_RE         = "{IEEE} Transactions on Rehabilitation Engineering"}



optics, lightwave and photonics
@STRING{IEEE_J_PTL        = "{IEEE} Photonics Technology Letters"}
@STRING{IEEE_J_JLT        = "{IEEE/OSA} Journal of Lightwave Technology"}



physics, electrons, nanotechnology, nuclear and quantum electronics
@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Letters"}
@STRING{IEEE_J_JQE        = "{IEEE} Journal of Quantum Electronics"}
@STRING{IEEE_J_JSTQE      = "{IEEE} Journal of Selected Topics in Quantum Electronics"}
@STRING{IEEE_J_ED         = "{IEEE} Transactions on Electron Devices"}
@STRING{IEEE_J_NANO       = "{IEEE} Transactions on Nanotechnology"}
@STRING{IEEE_J_NS         = "{IEEE} Transactions on Nuclear Science"}
@STRING{IEEE_J_PS         = "{IEEE} Transactions on Plasma Science"}



reliability
@STRING{IEEE_J_DMR        = "{IEEE} Transactions on Device and Materials Reliability"}
@STRING{IEEE_J_R          = "{IEEE} Transactions on Reliability"}



semiconductors, superconductors, electrochemical and solid state
@STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochemical and Solid-State Letters"}
@STRING{IEEE_J_JSSC       = "{IEEE} Journal of Solid-State Circuits"}
@STRING{IEEE_J_ASC        = "{IEEE} Transactions on Applied Superconductivity"}
@STRING{IEEE_J_SM         = "{IEEE} Transactions on Semiconductor Manufacturing"}



sensors
@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors Journal"}



VLSI
@STRING{IEEE_J_VLSI       = "{IEEE} Transactions on Very Large Scale Integration ({VLSI}) Systems"}






IEEE Magazines



@STRING{IEEE_M_AES        = "{IEEE} Aerospace and Electronics Systems Magazine"}
@STRING{IEEE_M_HIST       = "{IEEE} Annals of the History of Computing"}
@STRING{IEEE_M_AP         = "{IEEE} Antennas and Propagation Magazine"}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Magazine"}
@STRING{IEEE_M_CD         = "{IEEE} Circuits and Devices Magazine"}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits and Systems Magazine"}
@STRING{IEEE_M_COM        = "{IEEE} Communications Magazine"}
@STRING{IEEE_M_COMSOC     = "{IEEE} Communications Society Magazine"}
@STRING{IEEE_M_CIM        = "{IEEE} Computational Intelligence Magazine"}
CSEM changed to CSE in 1999
@STRING{IEEE_M_CSE        = "{IEEE} Computing in Science and Engineering"}
@STRING{IEEE_M_CSEM       = "{IEEE} Computational Science and Engineering Magazine"}
@STRING{IEEE_M_C          = "{IEEE} Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Computer Applications in Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Computer Graphics and Applications"}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Systems Magazine"}
@STRING{IEEE_M_DTC        = "{IEEE} Design and Test of Computers"}
@STRING{IEEE_M_EI         = "{IEEE} Electrical Insulation Magazine"}
@STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnology Review"}
@STRING{IEEE_M_EMB        = "{IEEE} Engineering in Medicine and Biology Magazine"}
@STRING{IEEE_M_EMR        = "{IEEE} Engineering Management Review"}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"}
@STRING{IEEE_M_IA         = "{IEEE} Industry Applications Magazine"}
@STRING{IEEE_M_IE         = "{IEEE} Industrial Electronics Magazine"}
@STRING{IEEE_M_IM         = "{IEEE} Instrumentation and Measurement Magazine"}
@STRING{IEEE_M_IS         = "{IEEE} Intelligent Systems"}
@STRING{IEEE_M_ITS        = "{IEEE} Intelligent Transportation Systems Magazine"}
@STRING{IEEE_M_IC         = "{IEEE} Internet Computing"}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Professional"}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
@STRING{IEEE_M_MW         = "{IEEE} Microwave Magazine"}
@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
@STRING{IEEE_M_NANO       = "{IEEE} Nanotechnology Magazine"}
@STRING{IEEE_M_NET        = "{IEEE} Network"}
@STRING{IEEE_M_PCOM       = "{IEEE} Personal Communications Magazine"}
@STRING{IEEE_M_POT        = "{IEEE} Potentials"}
CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power and Energy Magazine"}
@STRING{IEEE_M_PER        = "{IEEE} Power Engineering Review"}
@STRING{IEEE_M_PVC        = "{IEEE} Pervasive Computing"}
@STRING{IEEE_M_RA         = "{IEEE} Robotics and Automation Magazine"}
@STRING{IEEE_M_SAP        = "{IEEE} Security and Privacy"}
@STRING{IEEE_M_SP         = "{IEEE} Signal Processing Magazine"}
@STRING{IEEE_M_S          = "{IEEE} Software"}
@STRING{IEEE_M_SPECT      = "{IEEE} Spectrum"}
@STRING{IEEE_M_TS         = "{IEEE} Technology and Society Magazine"}
@STRING{IEEE_M_VT         = "{IEEE} Vehicular Technology Magazine"}
@STRING{IEEE_M_WC         = "{IEEE} Wireless Communications Magazine"}
@STRING{IEEE_M_TODAY      = "Today's Engineer"}






IEEE Online Publications



@STRING{IEEE_O_CSTO        = "{IEEE} Communications Surveys and Tutorials"}
@STRING{IEEE_O_DSO         = "{IEEE} Distributed Systems Online"}





--
EOF

